Simulation-Driven Balancing of Competitive Game Levels with Reinforcement Learning

The balancing process for game levels in competitive two-player contexts involves a lot of manual work and testing, particularly for non-symmetrical game levels. In this work, we frame game balancing as a procedural content generation task and propose an architecture for automatically balancing of tile-based levels within the PCGRL framework (procedural content generation via reinforcement learning). Our architecture is divided into three parts: (1) a level generator, (2) a balancing agent, and (3) a reward modeling simulation. Through repeated simulations, the balancing agent receives rewards for adjusting the level towards a given balancing objective, such as equal win rates for all players. To this end, we propose new swap-based representations to improve the robustness of playability, thereby enabling agents to balance game levels more effectively and quickly compared to traditional PCGRL. By analyzing the agent's swapping behavior, we can infer which tile types have the most impact on the balance. We validate our approach in the Neural MMO (NMMO) environment in a competitive two-player scenario. In this extended conference paper, we present improved results, explore the applicability of the method to various forms of balancing beyond equal balancing, compare the performance to another search-based approach, and discuss the application of existing fairness metrics to game balancing.

==> content/buffer.tex <==
We calculate for each agent $p$ at a given $t$ its win rate $wr_{p,t}$ from the number of all its won games $w_{p,t}$:
$$ wr_{p,t} = \frac{w_{p,t}}{N} $$

A game is considered to be balanced if all agents $P$ win the same number of games within $N$ simulations. This is expressed as $\frac{1}{P}$. $b_t$ is then formulated as:
$$ b_t = \sum^P_{p=1} |wr_{p,t} - \frac{1}{P}| $$

A value of 0 references to a perfect balanced state. The greater $b_t$ is the more imbalanced is the current level.

The reward $r_t$ is then calculated out of $b_t$ and $b_{t-1}$:
$$ r_t = b_{t-1} - b_t $$

If the agent improves the balancing state the reward will be positive, negative otherwise. For no impact on the balancing state the agent is given no reward (value 0).



\title{Balancing of competitive two-player Game Levels with Reinforcement Learning (Draft)\\

\thanks{This research was supported by the Volkswagen Foundation (Project: Consequences of Artificial Intelligence on Urban Societies, Grant 98555).}
}

\author{
\IEEEauthorblockN{Florian Rupp}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{University of Applied Sciences Mannheim}\\
Mannheim, Germany \\
Email: f.rupp@hs-mannheim.de}
\and

\IEEEauthorblockN{Manuel Eberhardinger}
\IEEEauthorblockA{\textit{Inst. for Applied Artificial Intelligence} \\
\textit{Stuttgart Media University}\\
Stuttgart, Germany \\
Email: eberhardinger@hdm-stuttgart.de}
\and

\IEEEauthorblockN{Kai Eckert}
\IEEEauthorblockA{\textit{Department of Computer Science} \\
\textit{University of Applied Sciences Mannheim}\\
Mannheim, Germany \\
Email: k.eckert@hs-mannheim.de}
}



\thanks{This research was supported by the Volkswagen Foundation (Project: Consequences of Artificial Intelligence on Urban Societies, Grant 98555).}

% regex to exclude Zotero file path from .bib: https://regexr.com/7a1l8 , file = \{.+\},




This paper proposes an architecture to balance tile-based levels with PCGRL. The idea is to reward a PCGRL agent for only altering a given playable level towards a balanced level.
A balanced level is a level where all agents with the same skill have the same win rate.
The architecture is depicted in Figure~\ref{fig:architecture}. It is separated into three parts: A level generator, a level balancing agent and a level playing simulation. In this research we came across much better results and faster training by splitting up the generation step into separated units instead of adding the balancing as constraint to the original PCGRL reward function (Section~\ref{sec:eval-swap}).
The controllable content generators introduced in~\cite{earle_learning_2021} are not applied thus, here the focus is on balanced levels and no diversity of balancing so far only. 

% short descr of gen agent
The level generator generates a playable level from random noise. Here we use PCGRL, however, other PCG methods will serve at this point comparable. The generator is trained separately before training the balancing agent. A detailed description is given in Section~\ref{sec:gen}. The generated level is then fed to the balancing agent.

% short descr of balancing agent
The core idea to balance the level is not to generate a new level but to modify the given level accordingly to fulfill the balancing goal. This could be e.g., to have the same win rate for all players in a game assuming all players have the same level of skill. Through the use of the exact same player agents to play the game it can be simulated accordingly. These player agents can be scripted or be trained machine learning models.
Each time step the balancing agent can decide to swap the positions of two selected tiles. If a swap was made (Section \ref{sec:swap}) the balancing reward is calculated by the environment. Therefore, the game level is played $n$-times in a simulation by player agents. The reward for the agent to learn from is then calculated out of the simulated balancing state (Section \ref{sec:reward}).

In this research we came across much better results and faster training by splitting up the generation step into separated units instead of adding the balancing as constraint to the original PCGRL reward function (Section~\ref{sec:eval-swap}).







%$b_t$ is calculated using the results from the player agent simulation step. In this step we let the player agents play the game level $n$-times.


%For the calculation of the balancing state $b_t$ we assign indices to the two players first where $p_1=0$ and $p_2=1$. For all $n$ simulations we count which player(s) won and save their player indices as winners $w_t$. The number of winners in the simulations are denoted as $wl_t$. Since draws are permitted, $n \le w_l \le 2n$. We calculate $b_t$ using Equation~\ref{eq:bt}:

%\begin{equation}
%\label{eq:bt}
%b_t = \frac{1}{wl_t} \sum^{w_t}_{i=0} w_{t,i}
%\end{equation}

%$b_t$ is defined in $[0,1]$ where 0.5 indicates both players won the same number of games, so the balance is maximal. The values 0 and 1 indicate a maximal unbalanced level where one distinct player wins every game. 0 indicates player 1 is only winning, 1 player 2. 

==> content/buffer2.tex <==
\section{Introduction}
 
The design of levels is a key concept when creating games. To keep players engaged, the balance between a challenging and enjoyable experience must be found. This is generally not an easy task, as it also depends on the skill and experience of the players~\cite{schreiber_game_2021}.
Furthermore, game levels for competitive multi-player games must be designed to be balanced towards equal initial win chances for all players. Imbalanced games will result in boredom or frustration and players will quit playing~\cite{andrade_dynamic_2006,becker_what_2020}.

To ensure balancing through the level design, game designers often rely on almost (point) symmetric map architectures. This can be seen in popular competitive esports titles such as League of Legends, DotA~2 or Starcraft~2, but also in other competitive tile-based games such as Advance Wars or Bomberman.
In addition to symmetrical levels, alternative approaches are also possible. Non-symmetrical levels offer more diversity and can create new ways for playful creativity to be entertaining and challenging.

For this work we frame the balancing task for levels as a procedural content generation (PCG) task. In previous works, several approaches have been proposed using (PCG) for level balancing, such as search-based approaches~\cite{togelius_search-based_2011,sorochan_generating_2022}, evolutionary algorithms~\cite{morosan_automated_2017,lanzi_evolving_2014,lara-cabrera_balance_2014,karavolos_using_2018,mesentier_silva_evolving_2019} or graph grammars~\cite{kowalski_strategic_2018}.
In this work, we introduce the balancing of tile-based levels with reinforcement learning (RL). Once a RL model is trained, it can generate levels fast and is less dependent on randomness compared to evolutionary methods. We apply RL for balancing by designing a reward function based on multiple simulation runs using scripted agents. While this approach becomes computationally intensive due to the simulations for each reward calculation, RL's advantage over \hl{other search-based approaches} lies in learning during training. This reduces the need for unnecessary simulations in the inference step, unlike e.g., evolutionary algorithms that start anew each time.
In addition, we develop our method to not be dependent on a single domain, as is the case with graph grammars or search-based approaches.

\begin{figure}
     \centering
        \includegraphics[width=2.8in]{content/images/res_water2.png}
    % \includegraphics[width=2.8in]{content/images/example1.png}
    \caption{
In our game environment, two players must forage for resources like food (dark green) and water (blue) to survive longest. By swapping the highlighted tiles (red), the trained model reached a more balanced game in simulated game runs. 
}
     \label{fig:gen-level1}
\end{figure}

Therefore, we use the procedural content generation via reinforcement learning framework (PCGRL)~\cite{khalifa_pcgrl_2020} which recently has been introduced for the generation of tile-based levels. Together with newly introduced swapping representations, our method can be viewed as a fine-tuning task to optimize a generated level towards a certain balance.
Our method is evaluated on the openly available Neural Massively Multiplayer Online (NMMO) environment~\cite{suarez_neural_2019} which has been designed for competitive multi-player research. We frame the problem as a resource gathering and survival game. Figure~\ref{fig:gen-level1} shows an example of how our method balanced a generated level (left) by swapping highlighted tiles (right). The code used in this research is available on Github\footnote{https://github.com/FlorianRupp/pcgrl-simulation-driven-balancing}.

Our contributions are:
\begin{itemize}
    \item A domain independent architecture for learning the automated altering of game levels towards a specified balancing with RL. 
    \item A novel swap-based representation pattern to frame the problem as Markov decision process.
    \item An experimental study to evaluate the proposed architecture compared to the original PCGRL method.
\end{itemize}

This paper is an extended version of the conference paper~\cite{rupp_balancing_2023}. We provide improved results, a detailed discussion on how existing fairness metrics can be transferred to game balancing, and a study of how this can be used for any balancing and not only equal balancing. Therefore, we revise the reward function and explain its derivation from the Statistical Parity metric~\cite{dwork_fairness_2012}.

The structure of this paper is as follows: We give a brief overview of related work~(\ref{sec:related-work}) and the background~(\ref{sec:background}). In Section~\ref{sec:method} the method is described and the implementation details in~\ref{sec:details} subsequently. Experiments and results are presented in~\ref{sec:experiments}, followed by an extended study on the generalized approach of an arbitrary balancing in~\ref{sec:extensions}. The discussion is in Section~\ref{sec:discussion}, the conclusion in~\ref{sec:conclusion}.

\section{Related work}
\label{sec:related-work}
% game balancing
For multiplayer \emph{game balancing}, several methods have been proposed in the past. One approach is the balancing through the configuration of game entities such as characters, weapons or items~\cite{schreiber_game_2021}. To do this, the games industry uses pipelines to extract data-driven insights from played games to adjust the balancing in a regular schedule\footnote{https://www.leagueoflegends.com/en-gb/news/dev/dev-balance-framework-update/}.

Evolutionary algorithms are further widely applied for game balancing.
Morosan et al. balance a real time strategy game (RTS)~\cite{morosan_automated_2017} and Sorochan et al. generate new and balanced units for an RTS game~\cite{sorochan_generating_2022}.
De Mesentier Silva optimize cards for the game Hearthstone~\cite{mesentier_silva_evolving_2019} to balance its metagame.
Another approach trains models with data from played games to replicate human behavior for automated balancing of entities~\cite{pfau_dungeons_2020}.

%A different method, especially in online games, are matchmaking algorithms~\cite{alman_theoretical_2017}. These methods assign which players play against each other or are in the same team and contributes to balancing by ensuring that the players' skill in a match is at a comparable level. Multiple works on this exist, however, many are based on a form of the Elo rating system~\cite{elo_rating_1978} used by the World Chess Foundation where a player's skill can be expressed by a single number. To integrate more information into the process and also improve player satisfaction, match making in~\cite{deng_globally_2021} is framed as an MDP to apply RL in a sequential task.  

The balancing of a level is furthermore influenced by its design. That refers to e.g., the position where game entities are located in relation to players' initial spawn position. As aforementioned, it is ensured with (point) symmetric map architectures in many games.
Contrary to the intended balancing the perception of players may differ. A survey concluded that a prevailing opinion among high experienced players is that only symmetrical levels can actually be balanced~\cite{togelius_controllable_2013}.

To automatically construct balanced levels with PCG, work has been introduced using evolutionary algorithms~\cite{lanzi_evolving_2014,lara-cabrera_balance_2014}. In contrast to this work, the fitness for balancing is evaluated rule based with heuristics or metrics. These metrics are either handcrafted or rely on a data-driven method using played games. In~\cite{karavolos_using_2018} this is extended with a convolutional neural network to predict game related information which are then used in the fitness function of an evolutionary algorithm to produce balanced levels. A different approach is the usage of graph grammars~\cite{kowalski_strategic_2018}. The balancing here is constructed by the rule-based placing of strategic game entities, which is, however, very dependent on the domain.

%In \cite{delaurentis_toward_2021} is a framework proposed to predict the balancing state based on played games with bots to balance a game.

% PCG
In this work, we focus on \emph{procedural content generation} for level generation, but the term PCG is also used in other applications such as the generation of game economies~\cite{rogers_using_2023}, rules~\cite{cook_mechanic_2013} or narratives~\cite{alvarez_tropetwist_2022}. PCG methods span over from dedicated algorithms~\cite{mojang_mincraft_2011}, search based methods~\cite{togelius_search-based_2011,lanzi_evolving_2014,lara-cabrera_balance_2014} up to the use of machine learning~\cite{summerville_procedural_2018} and deep learning~\cite{liu_deep_2021,giacomello_doom_2018,awiszus_toad-gan_2020,sudhakaran_prompt-guided_2023}. 
Once trained, machine \hl{learning based} methods can quickly generate content as needed, but they rely on having game levels already available from which a model can be learned. Therefore, when creating new games, these methods are usually not applicable efficiently.

In the games community, RL has been widely applied to \emph{play} games~\cite{silver_general_2018, vinyals_grandmaster_2019}, but recently, it has also been used for PCG~\cite{khalifa_pcgrl_2020,bontrager_learning_2021,gisslen_adversarial_2021,zakaria_procedural_2022}.
The framework we use and extend in this work is PCGRL~\cite{khalifa_pcgrl_2020}, utilizing RL for PCG tasks (cf. Section~\ref{sec:pcgrl}).
Zakaria et al. compare different deep learning-based PCG approaches for the puzzle game Sokoban, with PCGRL showing superior quality~\cite{zakaria_procedural_2022}.
There are already a \hl{few} methods which adapted the PCGRL method. In \cite{earle_learning_2021} controllable content generators were introduced, where users control the generated content with additional constraints, such as e.g., the number of players.
We do, however, not compare our method with it, as our objective is a balanced level only.
Other approaches use evolutionary strategies on top of the PCGRL framework to achieve more content diversity~\cite{khalifa_mutation_2022} or adapted the method for 3D environments \cite{jiang_learning_2022-4}.


\section{Background}
\label{sec:background}
\subsection{The PCGRL framework}
\label{sec:pcgrl}
In this work, we use the PCGRL \cite{khalifa_pcgrl_2020} framework for level balancing.
In PCGRL, PCG is formulated as a sequential decision-making task to maximize a given reward function, where semantic constraints can be expressed and thus, no training data is needed. To apply RL, the PCG problem is framed as a Markov decision process (MDP).

Therefore, PCGRL introduces three different MDP representations for level generation. 
We will introduce three new swap representations based on the existing representations. Later we argument that they are a better fit to alter game levels to improve e.g., the balancing state. The original representations in PCGRL are: 

\paragraph{Narrow} This representation randomly selects a tile in the grid and the agent only needs to decide what type of tile should be placed on the selected position. This has a small action space since it only consists of the different types of tiles. 

\paragraph{Turtle} The \emph{turtle} representation allows the agent to move on the map and then to decide what type of tile to put on the current position. The advantage to the narrow representation is that the agent is not restricted to the randomly assigned position and therefore can learn where to move next.

\paragraph{Wide} In the \emph{wide} representation the agent is given full control of the level generation process as the agent can decide which tile of the whole grid should be changed. This increases the action space greatly thus every position of the grid multiplied by the number of tiles represents an action. This is the most human-like representation as the agent can change everything directly according to a plan it has constructed.

\subsection{The Neural MMO Environment}
\label{sec:nmmo}
As basis for our experiments, we use the NMMO environment~\cite{suarez_neural_2019}. The NMMO environment is a Massively Multiplayer Online Battle Royal inspired multi-agent RL environment for research.
It simulates a tile based virtual world where agents must forage for resources to survive and be prepared for fights with other agents. All actions of the agents are processed simultaneously per time step. The agent which survives the longest wins the game.
The agent's state is represented by its position as well as its current health, food, and water level.


In this paper, we focus on the balancing in the PCG process of the game map. To apply and evaluate our method, we simplify the win condition and frame the game as a forage survival game. Therefore, we disable the combat system and limit map tiles to the types of grass, forest, stone, and water. The agent cannot move on stone nor water tiles. Forest and water are resources \hl{that} the agent can gather. A detailed overview of the tiles and their behaviors is given in Figure~\ref{fig:tile-descr}. When moving on a forest tile, it is consumed automatically as food and refills the agent's food indicator. In the process the forest tile changes to the state \emph{scrub}. Scrub tiles cannot be consumed, however, there is a probability of 2.5\% per time step to respawn and transit back to the forest state.
To refill the agent's water indicator\hl{,} it must simply step on an adjacent tile. Water tiles are not depleted. If one of both resource indicators are empty the agent loses a fixed amount of health per step. If the agent's health indicator drops to zero, the agent dies. An agent can restore health having water and food indicators over 50\%. 

\begin{figure}
     \centering
     \includegraphics[width=0.7\linewidth]{content/images/tiles.png}
     \caption{Description of the NMMO tiles.}
     \label{fig:tile-descr}
\end{figure}

For this research we frame the win condition equally for both agents. The agent which completes one of two goals first wins:
\begin{itemize}
    \item Collect five food resources.
    \item Last agent standing: Not starved nor died of thirst.
\end{itemize}

In this introductory research, we fix the map size to a grid of 6x6 tiles and two players to speed up the experiments and to keep the results interpretable by human evaluators. Furthermore, the smaller grid size limits the available space and resources which reinforces the competitive race of the agents. This competitive race is to be balanced in this paper.


\section{Method}
\label{sec:method}
\subsection{Balancing architecture}
\label{sec:architecture}

\begin{figure*}
  \centering
  \includegraphics[width=0.9\linewidth]{content/images/balancing-architecture.png}
  \caption{Description of the balancing architecture. It is separated into three units: A level generator, a level balancing agent and a level playing simulation. In the latter, the game is simulated by playing it $n$-times with player agents. The reward $r_t$ for training the balancing agent is calculated out of the balancing states $b_t$ and $b_{t-1}$ from the simulations.}
  \label{fig:architecture}
\end{figure*}

This paper proposes an architecture to balance tile-based levels with RL. The idea is to reward a PCGRL agent for only altering a given playable level towards a balanced level.
A balanced level is a level where all player agents with the same skill have the same win rate.
We only focus on game balance through level design, which excludes balancing a sequence of levels or different play styles for instance.
The architecture is depicted in Figure~\ref{fig:architecture}. It is separated into three parts: a level generator, a balancing agent and a playing simulation. 

% short descr of gen agent
The level generator constructs a playable level from random noise which is then fed to the balancing agent. In this work we use PCGRL for the generator, however, other PCG methods will serve at this point comparable. The generator is trained separately before training the balancing agent.

% short descr of balancing agent
The core idea to balance the level is not to generate a new level but to modify the given level accordingly to fulfill the balancing constraint.
Each time step the balancing agent can decide to swap the positions of two selected tiles. If a swap (Section \ref{sec:swap}) was made, the level is played $n$-times in a simulation by player agents. Subsequently, the balancing agent is rewarded based on how this action influenced the balancing state in simulations (Section \ref{sec:reward}). This is inspired from the idea of simulation-based fitness functions in~\cite{togelius_search-based_2011}.

More details are given in the implementation details~(Section~\ref{sec:details}).


\subsection{Swap-based representation pattern}
\label{sec:swap}
To formulate the problem of PCG with RL as MDP three representations have been introduced in \cite{khalifa_pcgrl_2020}. In all of them the agent can decide to replace a tile at a distinct position. This method, however, may result in unplayable levels at a time step. Furthermore, to move the position of e.g., a player tile somewhere else, the agent would need to remove the player tile first before creating it at a different position. In this time step the level would not be playable for the player agents and thus, no reward could be computed in the simulation step. Additionally, the agent would get a negative reward first due to the number of players is now invalid. The subsequent creation at a different position under the previously given negative reward is hard to learn for RL agents.

For this reason, we introduce a swapping-based representation pattern. In these representations the agent can decide to swap the positions of two tiles per time step.
Not adding or removing tiles entirely is a more robust approach to ensure level playability.

There might be, however, game domains where multiple tiles have a semantic connection e.g., multiple river tiles construct a river. Swapping these tiles around can break playability. Therefore, we suggest in the balancing step to feed unplayable levels back to the generator to fix it again.
This repair is similar to the level fixing seen in~\cite{siper_path_2022}, but it would also involve an additional increase in computational effort.

In this work we demonstrate the power of swapping with a simpler domain where no semantic relations of multiple tiles exist. In addition, swapping tiles ensures that the old level isn't simply generated from scratch since that's the job of the level generator.
Swapping two tiles of the same type has no effect on balancing. Thus, we prevent these swaps to reduce computational intensity. In these cases, the agent is rewarded with 0.
Therefore, we extend the narrow, turtle and wide representations~\cite{khalifa_pcgrl_2020} with a swapping mechanism:

\paragraph{Swap-Narrow} As in PCGRL the agent observes the tiles in the environment one-hot encoded. At each time step two random tile positions are presented to the agent, and it can decide to swap the tiles or not. The agent's little position control results in in a very small action space $A$ with only two actions: swap or do not swap. $A$ is therefore $A=[2]$.
\paragraph{Swap-Turtle} Starting at two random positions the agent can decide to swap the tiles at the current positions in each time step. If no change is made it can decide to which adjacent tile to move next. As in the original PCGRL, staying in one position and not changing a tile is not an option. The observations are in a one-hot encoded format as well. $A$ is therefore $A=[4,4,2]$ which results in 32 possible actions.
\paragraph{Swap-Wide} In this representation the agent sees the whole level and can freely determine the tile positions and whether to swap it. The observations are provided one-hot encoded. It can be interpreted as looking at the whole level and then decide what to move where. A drawback here is the large action space since it scales twice with the grid width $w$ and height $h$. $A$ is therefore $A=[w,h,w,h,2]$. In the case of a square grid shape as in this work with a size of 6, $A$ has 2592 possible actions.

\subsection{Reward design}
\label{sec:reward}
For the successful training of a RL agent, the reward function is crucial. Heuristic approaches for the evaluation of balancing have been introduced in~\cite{lanzi_evolving_2014,lara-cabrera_balance_2014}. These approaches, however, include domain specific information and are thus not transferable. To address this shortcoming, we propose the use of a more generic, game domain independent reward function only relying on how often each player wins. In addition, we require the game to have at least one winner at its end. Since draws also provide information about the balancing state, our reward function must handle this as well.

To measure the balancing appropriately, we are inspired by fairness metrics from the fair machine learning community. A survey of common metrics used in that field is provided in~\cite{makhlouf_applicability_2021}. The Statistical Parity metric~\cite{dwork_fairness_2012} is one of them and often used to measure fairness between two groups. The fairness for two groups $G=1$ and $G=2$ is considered as fair if the conditional probability of the same outcome $\hat{Y}$ for both groups is the same, as seen in Eq.~\ref{eq:stat-parity}. 

\begin{equation}
\label{eq:stat-parity}
P(\hat{Y}\,|\,G = 1) = P(\hat{Y}\,|\,G = 2)
\end{equation}

In this work, we transfer this definition of fairness to the domain of game balancing. 
In the context of the Statistical Parity, the two groups represent the two players\hl{,} and we want to optimize their win rates.
%, cf. $P(win \,|\, player = 1) = P(win \,|\, player = 2)$. 
However, the direct use of Eq.~\ref{eq:stat-parity} is not applicable to RL since it requires a function that rewards the agent with positive or negative incentives per time step $t$. In addition, an intermediate reward design which compares $t$ to $t-1$ has shown good results in PCGRL.
First, we therefore define the win rate $w_{p_it}$ per player $p_i$:
\begin{equation}
\label{eq:bt}
w_{p_it} = P(w_t\,|\,p = i)
\end{equation}
$w_{p_it}$ is then inferred from the data from the $n$-runs of the player agent simulations per step. This could be viewed as a sampling from the actual win rate distribution (cf. Section~\ref{sec:simulation} and Fig.~\ref{img:balancing}).
Second, in this extended paper we additionally want to make the reward design configurable to a certain balancing state $b$ and thus rewrite the balancing calculation $b_t$ as:

\begin{equation}
\label{eq:b}
b_t = |\, w_{p_1t} - b \,|
\end{equation}

%The balancing state $b_t$ is the absolute value of the deviation of a player from $b$.
Due to the use of the absolute value, $w_{p_it}$ of both players could be used in Eq.~\ref{eq:b} as their values describe probabilities which sum up to 1.
%We design the reward function to reward the agent for improving the balancing state $b_t$ in time step $t$ in comparison to $b_{t-1}$.
$b_t$ is defined in $[0,1]$ as well where 0 indicates $b_t$ corresponds exactly to $b$; 1 indicates the maximal deviation from $b$. In the example where an exact balance between both players is desired ($b=0.5$), $b_t=1$ indicates one distinct player wins every game.
With $b_t$ in this range, there is flexibility to configure toward which player the game should be balanced to.
Finally, the reward $r_t$ is: 
\begin{equation}
\label{eq:reward}
r_t = b_{t-1} - b_t  + \alpha
\end{equation}

To additionally reward the agent, a reward $\alpha$ is given if $b_t$ is exactly $b$. Otherwise, $\alpha$ is 0. If $\alpha>0$ the episode always ends as $b_t=b$.
As a result, the reward will be positive if the agent improves the balancing state, negative otherwise. For no impact on the balancing state the agent receives no reward (value 0). Applying this reward design, the RL agent is gradually incentivized to reduce the absolute difference from current balancing state to the intended one.


\section{Implementation details}
\label{sec:details}
\subsection{Level generator}
\label{sec:gen}

The task of this unit is to generate playable levels for balancing. In this work, the generator is a model trained using the PCGRL framework.

The reward for the training process is designed to reward the agent to
\begin{itemize}
    \item have exactly two players and
    \item create a valid path between both players.
\end{itemize}

To guarantee the direct competition, the latter constraint ensures that both players have access to the same area of the game level. Additionally, this prevents single players being locked within stone walls.

The NMMO environment uses by default PCG to generate random levels, however, the players' spawn positions are randomly determined when the game starts. Nonetheless, the spawn positions are crucial for balancing and thus, should be possible to be aware of and to influence by the balancing agent. For this reason, a player tile is integrated in the level generation process representing the positions.

If a valid path between both players exists the agent receives a positive reward, a negative otherwise. Additionally, each step the agent is rewarded with the difference of players there are and should be (similar to \cite{khalifa_pcgrl_2020}). We achieve the best results using the \emph{wide} representation. An episode ends when both constraints are met, or the agent exceeds a fixed number of permitted steps or changes.

After training, the model can produce levels satisfying the given constraints in 98,7\% levels out of an evaluation sample of 5000. The generated levels achieve a maximum diversity at 100\%, so no two levels are completely identical. An example of a generated level is shown in Figure~\ref{fig:gen-level1}~(left) and a tile legend is given in Figure~\ref{fig:tile-descr}.

The yielded levels are then passed on to the balancing agent. Level generation at this step is done until the agent produced a valid level fulfilling the constraints to ensure the balancing agent receives playable levels only.

%\begin{figure}[!t]
%  \centering
%  \label{img:genagent}
%  \includegraphics[width=2.5in]{content/images/pcgrl_map.png}
%  \caption{A playable, not yet balanced game level for the NMMO environment generated with PCGRL. Exactly two players exist which are connected. The colored tiles represent the NMMO tiles: blue=water, grey=stone, light green=grass and, dark green=forest. Additionally the spawn positions of the players are represented with the face icon.}
%\end{figure}


\subsection{Balancing agent}
\label{sec:balancing}
The balancing agent is the core component of the architecture in Figure \ref{fig:architecture}. We model the agent as PCGRL agent which can decide to alter a previously generated game level per time step. To support this process, we use swapping representations.
The reward is calculated out of the results of a simulation of the balancing state (Section \ref{sec:reward}).

The observation is the current level one-hot encoded. In detail, this depends on the chosen representation. As RL algorithm, we apply PPO (proximal policy optimization)~\cite{schulman_proximal_2017}.
An episode ends when the level is either balanced, or a fixed number of steps or changes is exceeded. In PCGRL, the number of changes allowed is determined relative to the grid size (cf. change percentage). As in the original PCGRL we use a change percentage of 20\%. We set the value for the number of allowed steps within an episode to 100.

\subsection{Player simulation}
\label{sec:simulation}
To calculate $b_t$ for the reward (Section~\ref{sec:balancing}) we run a simulation $n$-times of player agents playing the game.
The player agents can be any solution which can simulate a player's behavior at a required quality. In this work we use the scripted \emph{Forage}-agent for the NMMO environment which is publicly available\footnote{https://github.com/NeuralMMO/baselines}. The usage of scripted agents provides the benefit of a deterministic behavior at any time step. If the agent's water or food indicator drops below a certain threshold it looks for the next available resource of that type to refill it.
At this point, however, the application of trained agents with e.g., RL, different skilled or types of agents is feasible as well. See the discussion~(Section~\ref{sec:discussion}) for further information.

Despite running the simulation with the same player agents, winners may differ each pass. This is because of probabilistic mechanics making games interesting such as rolling dices or the respawn of resources at a certain probability. A player may win with luck, but when playing many times, skill should make the difference. The question is then, how often must a simulation be run to minimize the noise of probability? \hl{Since the simulations are computationally intensive}, it is of interest to find the number of minimal runs where win rates vary at an acceptable level.

We approach this by investigating how much the win rates $w_n$ of a specific number of simulations $n$ differ on average from $n-2$. Only even values for $n$ are applicable since otherwise a balanced game is not possible. Therefore, we run the simulation on a sample of size $s=500$ levels up to a number of $N=30$ times and compare how win rates for $n$ fluctuate on average in comparison to $n-2$. The average deviation~$\mu_n$ of a distinct $n$ is expressed with: $\mu_n = \frac{1}{s} \sum^{N}_{n=0} | w_n - w_{n-2} |$ and its course is depicted in Figure~\ref{img:balancing}. In addition, the standard deviation is given with $\sigma$ and $2\sigma$. It is clear that the larger $n$ is, the smaller $\mu_n$ is. To determine an appropriate $n$ we set the threshold: $\mu_n + \sigma < 0.05$. For this game with the configured number of players, this applies to $n \ge 14$. Therefore, we use $n=14$ in this work.


\begin{figure}[!t]
  \centering
  \includegraphics[width=3.1in]{content/images/balancing_metric.png}
  \caption{How many times $n$ should we run the simulation to approximate the balancing state? We figure that out by calculating the mean deviation $\mu_n$ of win rates from $n-2$ to $n$ for the investigation of fluctuations in win rates.}
  \label{img:balancing}
\end{figure}

This method can be used to determine $n$ for any domain.


\section{Experiments and Results}
\label{sec:experiments}

We evaluate our architecture in several steps: \hl{First}, we sample a fixed data set of levels to use for direct comparison with the generator. \hl{Second}, we compare the balancing performances of the three introduced representations with the original PCGRL method as a baseline~(\ref{sec:eval-swap}). To generate balanced levels with the original PCGRL method, we integrated the balancing constraint into the reward function.

Subsequently, we investigate on the levels the models created~(\ref{sec:gen-levels}) and examine which tiles the models swapped in the level altering process~(\ref{sec:impact}). The latter can provide insights about which tiles actually influences the balancing.

\subsection{Performance overall}
\label{sec:eval-swap}
We compare the performance of the swap representations among themselves and in contrast to the original PCGRL as baseline\footnote{Only the narrow representation is shown here; the other two yield similar results.}. For direct comparison all models have been trained the same amount of 200k training steps resulting in 970 updates of the policy.

For the evaluation we create a data set of 1000 levels with our PCGRL generator. This data set is then used for all four models for evaluation.
First of all, \hl{we investigate the} distribution of initial balancing states of the levels in the data set (see Figure~\ref{fig:init-balancing}). Important to mention here is the non-equal distribution. Except the states 0 and 1 the levels seem to be normal distributed around the state of 0.5, indicating both players won equally often. A share of 13.6\% of levels is initially balanced. However, peaks towards maximally unbalanced levels at the outer edges of the distribution can be observed. Maximally unbalanced levels make up 26.6\% in the data set.

\begin{figure}[!t]
  \centering
  \includegraphics[width=2.9in]{content/images/hist_initial_balancing.png}
  \caption{Distribution of the initial balancing states based on the players' win rates in the generated data set of 1000 levels. We use this data set to compare the different representations.}
  \label{fig:init-balancing}
\end{figure}

To evaluate the performance of the balancing method we compare the balancing state before and after per representation. A general overview is given in Table~\ref{tab-overview}. A histogram of the balancing improvement is depicted in Figure~\ref{fig:repr-compare}. 

The performance of all three swap representations is at comparable quality. Each representation managed to improve the share of balanced levels significantly. The swap-narrow and swap-wide representations perform slightly better towards balancing in contrast to swap-turtle.
The plain PCGRL narrow representation also improved the share of balanced levels, however, with 36.7\% this share is smaller compared to the swap representations. Additionally, a proportion of 38.8\% of the levels are in an unplayable state at episode end~(Figure~\ref{fig:narrow-pcgrl}); whereas our methods result in 100\% of playable levels in all cases on this domain.
In all results, however, remain unbalanced levels. The biggest share remains for the balancing states 0 and 1.
For representations with a higher proportion of balanced levels, the average episode lengths are shorter. This is because levels that remain unbalanced will max out the episode length.

%\begin{figure}[!t]
 % \centering
 % \includegraphics[width=3.5in]{content/images/repr_compare.png}
 % \caption{Comparison of balancing distributions of the balancing states before and after the balancing method per each representation. The same data set of of 1000 levels is used each time.}
%  \label{fig:repr-compare}
%\end{figure}



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
          \centering
          \includegraphics[width=\textwidth]{content/images/repr_compare.png}
          \caption{\normalfont Swap representations}
          \label{fig:repr-compare}
     \end{subfigure}
     \vspace{\fill}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/images/result_narrow_pcgrl.png}
         \caption{\normalfont Original PCGRL (narrow)}
         \label{fig:narrow-pcgrl}
     \end{subfigure}
    
          \caption{Comparison of balancing state distributions before and after the balancing process per each representation using the data set of 1000 levels (Figure~\ref{fig:init-balancing}). The swap representations (a) are compared to the original PCGRL implementation directly~(b).}
     \label{fig:repr-compare}
\end{figure}



%\begin{table}[]
%\centering
%caption{Performance overview of the representations. Initially balanced levels were not taken into account.}
%\label{tab-overview}
%\begin{tabular}{@{}lllll@{}}
%\toprule
%                        & Swap-narrow  & Swap-turtle   & Swap-wide    & PCGRL        \\ \midrule
%Balanced (\%)           & \textbf{48.1}   & 42.5          & \textbf{48.1}  & 30.4    \\
%Improved (\%)           & 63.3         & 56.8          & \textbf{64.1}    & 36.7      \\
%Playable (\%)           & 100          & 100           & 100            & 61.2      \\
%Avg. changes            & 4.6$\pm$1.9  & 4.7$\pm$1.9   & 4.9$\pm$1.9  & 5$\pm$1.8    \\
%Avg. ep. length         & 11.3$\pm$6.1 & 25.4$\pm$17.7 & 14.1$\pm$7.9 & 15$\pm$7.9   \\
%Size action space       & 2            & 32            & 2592         & 10           \\
%Compute time (h)       & \textbf{52}   & 40              & 33            &  \\
%\bottomrule
%\end{tabular}
%\end{table}


\begin{table}[btp]
\caption{Performance overview of the representations. Initially balanced levels were not taken into account.}
\begin{center}
\begin{tabular}{l|l|l|l|l}
                        & {\textbf{S-narrow$^{\mathrm{*}}$}}  & {\textbf{S-turtle$^{\mathrm{*}}$}} & {\textbf{S-wide$^{\mathrm{*}}$}} & {\textbf{PCGRL}}   \\
\hline
Balanced (\%)           & \textbf{48.1}   & 42.5          & \textbf{48.1}  & 30.4    \\
Improved (\%)           & 63.3         & 56.8          & \textbf{64.1}    & 36.7      \\
Avg. changes            & 4.6$\pm$1.9  & 4.7$\pm$1.9   & 4.9$\pm$1.9  & 5$\pm$1.8    \\
Avg. ep. length         & 11.3$\pm$6.1 & 25.4$\pm$17.7 & 14.1$\pm$7.9 & 15$\pm$7.9   \\
Size action space            & 2            & 32            & 2592         & 10           \\
\multicolumn{2}{l}{} \\
\multicolumn{4}{l}{$^{\mathrm{*}}$Swap representations are abbreviated with S.}
\end{tabular}
\label{tab-overview}
\end{center}
\end{table}


\subsection{Generated levels}
\label{sec:gen-levels}
Figure \ref{fig:gen-level1} and \ref{fig:gen-levels} give examples of the different types of generated levels taken from the samples in Section \ref{sec:eval-swap}. Figure \ref{fig:res-perfect} is an example where the balancing agent altered the given level to a balanced level by swapping only one tile. By swapping the highlighted grass tile with the rock tile the path to the resource (forest) tiles is now blocked. This results in a more equal availability of food resources for both players. In Figure \ref{fig:gen-level1} the agent balanced the level from an initial balancing state of 0.3 to 0.5. By swapping the marked water tile to a more central position for both players, the balancing is improved. In Figure \ref{fig:res-failed} the agent failed to balance the initial level with $b_0=0$. The balancing process terminated after the maximum of permitted changes has been reached. In the end $b$ is still 0.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.41\textwidth}
         \centering
         \includegraphics[width=58mm]{content/images/res_perfect2.png}
         \caption{\normalfont The agent balanced a maximally unbalanced level (0) towards a balanced level (0.5) by swapping one tile.}
         \label{fig:res-perfect}
     \end{subfigure}
      \vspace{\fill}
     \begin{subfigure}[b]{0.41\textwidth}
         \centering
         \includegraphics[width=58mm]{content/images/res_nochange2.png}
         \caption{\normalfont The agent could not change the initial balancing of 0. Generation stopped after a permitted number of changes has been exceeded. Since several tiles have been swapped, they are not highlighted for the sake of visualization.}
         \label{fig:res-failed}
     \end{subfigure}
    
    \caption{Examples of altered levels by the balancing agent. The left column shows generated levels before balancing. The right level is the result after the balancing process. Swapped tiles are indicated by red frames.}
     \label{fig:gen-levels}
\end{figure}

\subsection{Impact of tiles on balancing}
\label{sec:impact}
The analysis of the actual swaps a model made gives insights on its behavior. Thus, we showed the model could improve the balancing state of the given levels, we can further argue that swaps made by the model have impact on the balancing. In reverse, we can conclude from this behavior which tiles in the game have most impact on balancing.

For comparison, we calculate per swap pair the relative differences of frequencies of random swaps with the ones from the models. Therefore, these frequencies are factorized with the inverse probabilities of total tile occurrences in the data set. Due to swapping the same tile types is prohibited by the representations, ten different combinations are possible. This is depicted in Figure~\ref{fig:swaps}.
The figure shows the three representations have different behaviors; however, they agree in particular points. Most impact has the swapping of forest with stone tiles, second the swap of forest with water tiles. This makes sense in the context of the resource gathering win condition. Relocating the resource tiles forest or water will likely affect the balancing state thus, they are included in the win condition.
A stone field can be used to block the way for players. Due to this, the swapping of forest with stone tiles has an additional powerful impact.
Surprisingly swapping players' spawn positions is not a favored action in all cases.


\begin{figure}[!t]
  \centering
  \includegraphics[width=3.5in]{content/images/swap-analysis2.png}
  \caption{Comparing the swapped tiles by the model per representation on the generated 1000 levels. The comparison is made in relation to the inverse tile type distribution of all levels. This shows the difference to random swapping.}
  \label{fig:swaps}
\end{figure}


\section{Extended study on general improvements and balancing with a varied target balance}
\label{sec:extensions}

In Section~\ref{sec:experiments} we focused on a balancing where both players win equally often. This study extends the paper's core idea to demonstrate that this method \hl{can optimize} given levels towards arbitrary balancing values as well. Furthermore, the performances of the trained models are improved.

\subsection{Improvement of results}
\label{sec:improvements}

To improve the results from Section~\ref{sec:experiments}, we addressed two issues:
First, previously both players' spawn positions were represented by the same type of tile, making it impossible for the model to distinguish.
For this reason, we are now assigning different tile representations to each spawn position, as our previous research has shown that these affect balancing.
The different encoding of both positions adds more information and thus slightly increases the observation space, but the action space remains the same. \hl{Training using identical conditions as described in Section~}\ref{sec:experiments}\hl{ improves the previous results to 65.6\% of levels achieving balance for $b=0.5$.
Second, we improved the performance of our code, reducing computation time. As a result, training became more efficient, allowing for more updates (10k) to the model's policy within the same time frame.}

In the results of the experiments in Table~\ref{tab-overview}, the best model could balance 48.1\% and could improve 64.1\% of the levels towards a balancing of 0.5. In this extended work, we improve the proportion of balanced levels to 68.0\% compared to the baseline (Table~\ref{tab:unbalancing}). \hl{The extended training could additionally lead to a slight improvement in performance (2.4 percentage points).}
Levels where the model could at least improve towards the desired balancing are improved to a proportion of 88.9\%. A level is considered improved if the balancing is equal or comes closer to the desired state.

\subsection{Balancing with different target values}
\label{sec:unbalancing}
With this experiment series we expand the previous research towards also training models to generate levels which are not balanced equally for both players. This shows that our method is capable of balancing levels to a distinct value in general.

Therefore, we use the adjusted reward function (Eq.~\ref{eq:reward}) which is configurable with a parameter $b$ towards a desired balancing. We investigate this by training six different models in tenth increments of possible values for $b$ in the interval $[0,0.5]$. As it performed best according to the previous results we use the swap-wide representation in combination with the improvements from Section~\ref{sec:improvements}. We refrain from implementing a single but controllable approach as in~\cite{earle_learning_2021}, as we experiment with different parametrizations of the reward function only. Applying controllable RL would mean an adaption of the previously defined MDP, making a direct comparison with the previous results difficult.
To evaluate all models, we use the same level data set from Section~\ref{sec:eval-swap} to ensure comparability. An overview of the results is given in Table~\ref{tab:unbalancing}.
%Figure~\ref{fig:unbalancing}.

For all values of $b$, a significant improvement of the respective balancing state can be observed (blue). The performance, however, differs depending on $b$. For $b \geq 0.3$ the proportion of levels with the desired balancing is even higher than the baseline from the previous experiments. For the value 0 indicating levels being heavily balanced towards one specific player the performance is slightly worse than the baseline. In all cases, however, the models could improve the balancing towards the given value significantly.

Creating diverse content is of interest when implementing a PCG method~\cite{togelius_search-based_2011}. For all generated levels per model, we therefore evaluate their diversity through matrix comparisons. We determined for each $b$ a content diversity of 100\% of the balanced levels. For more information regarding the asymmetries of levels see Section~\ref{sec:asymmetries}.
%This \hl{work} aims to generate asymmetrical yet balanced levels. To evaluate this, we checked all levels for each model, considering both diagonals as well as the vertical and horizontal axes. None of the levels created had any form of symmetry.
%Both, the checking of diversity and symmetry are solutions at the value layer, however, not at the semantic one. There may be levels that are semantically the same e.g., if only a few tiles are different, which have no influence on the game. This process, however, cannot be easily automated.

\begin{table}
    \centering
    \caption{Performance overview of six swap-wide models trained to optimize different balancing values $b$ across the interval $[0,0.5]$ of the balancing metric (cf. Section~\ref{sec:reward}). All values are expressed as percentages.}
    \begin{tabular}{c|c|c|c|c}
         $b$ &  \textbf{Balanced to $b$}&  \textbf{Improved toward $b$} & \textbf{Initial $=b$} & \textbf{Baseline} \\ \hline
         0.0&  36.1&  71.1&  8.6& -\\
         0.1&  35.1&  73.5&  7.2& -\\
         0.2&  42.9&  76.3&  6.4& -\\
         0.3&  54.6&  77.9&  11.4& -\\
         0.4&  60.7&  81.4&  12.0& -\\
         0.5&  \textbf{68.0} &  88.9&  15.6& 48.1\\
    \end{tabular}
    \label{tab:unbalancing}
\end{table}


%\begin{figure*}[!t]
%  \centering
%  \includegraphics[width=0.75\linewidth]{content/images/unbalancing_overview.png}
%  \caption{Performance overview of eleven swap-wide models trained to optimize different balancing values $b$ across the interval $[0,1]$ of the balancing metric (cf. Section~\ref{sec:reward}). The plot shows the improvement of the proportion of the levels which are initially in the desirable state (red) to the proportion after the balancing proceeding (blue). The green line represents the proportion of levels where the models could at least improve the balancing value towards the desired goal. For all results, levels which are already in the desired balancing state have been filtered out. As a baseline, the previous result from Section~\ref{sec:experiments} is shown~(orange).}
%  \label{fig:unbalancing}
%\end{figure*}

%\section{Extended study on adding more player agents}

%\subsection{Reward design for n-players}
%\begin{equation}
%\label{eq:new-bt}
%wr_{p,t} = \frac{1}{wl_t} \sum_{i=1}^{w_{p,t}} w_{p,t,i}
%\end{equation}


%\begin{equation}
%\label{eq:new-bt}
%b_t = \sum_{p=1}^{P} | wr_{p,t}-\frac{1}{P} |
%\end{equation}

%\subsection{Level generator for N players}

%\subsection{Direct comparison of the old reward function with new function}

%\subsection{Experiments and Results}


\subsection{Comparison with other search-based approaches}

To further evaluate our method in comparison to another search-based method, we compare its performance against a hill climbing approach. Therefore, we run the hill climbing approach and the models listed in Table~\ref{tab:unbalancing} on the dataset of 1000 generated levels and compare the run times\footnote{We use for all experiments an AMD EPYC processor with 2.6 GHz.} at inference.

Our hill climbing implementation operates as follows: During each iteration, the method randomly selects an action from the swap-wide representation's action space (similar to the swap-narrow representation). In contrast, the hill climbing agent must swap at each iteration since there is no model to predict this behavior. We utilize the same reward function to evaluate the balancing (Eq.~\ref{eq:reward}) as when using PCGRL. The execution terminates either when the desired balancing is achieved or when a maximum of 1000 iterations is reached. Positive rewards trigger the transition to the next iteration with the new map state, while negative rewards revert the map state to the previous one.
Levels initially complying the given balancing constraint are not considered.

Table~\ref{tab:execution-time} shows that, on average, execution times are notably faster compared to the hill climbing method across all values of $b$ for PCGRL.
Both methods exhibit their swiftest execution for $b=0.5$, with performance gradually declining towards $b=0.0$. Achieving win probabilities favoring a selected player appears to pose a greater challenge within this environment. The decreasing computation times observed for PCGRL from $b=0.0$ to $b=0.5$ also mirror the findings in Table~\ref{tab:unbalancing}, where $b=0.5$ showcases the best performance. In addition, PCGRL demonstrates greater consistency in execution times for content creation, contrasting with the hill climbing method, which displays significantly higher and more dispersed standard deviations.


%\begin{table}
%    \centering
%    \caption{Comparison on execution times with a hill climbing approach. All values are given in seconds.}
%    \begin{tabular}{c|cc|cc}
%         $b$ &  \multicolumn{2}{l|}{\textbf{PCGRL S-wide}} &   \multicolumn{2}{l}{\textbf{Hill climbing (swap)}}  \\ %\hdashline
%            &  Avg. & Std.  &  Avg. & Std.  \\ \hline
%         0.0& 10.59 & 4.37 & 45.29 &  52.81 \\
%         0.1& 10.57 & 4.29 & 40.88 &  55.89 \\
%         0.2& 10.10 & 4.23 & 26.37 &  28.56 \\
%         0.3&  9.42 & 4.25 & 24.66 &  50.80 \\
%         0.4&  8.99 & 4.06 & 26.11 &  89.96 \\
%         0.5&  8.37 & 4.07 & 11.47 &  9.68  \\
%    \end{tabular}
%    \label{tab:execution-time}
%\end{table}


\begin{table}
    \centering
    \caption{Performance comparison of PCGRL with hill climbing approaches for optimizing different balancing values $b$. All values are expressed as percentages.}
    \begin{tabular}{c|c|c|cc}
          &  \textbf{PCGRL} &   \multicolumn{3}{c}{\textbf{Hill climbing}}  \\ 
          $b$  & S-wide & S-narrow & narrow & unplayable\\
         \hline
         0.0& \textbf{36.1} & 30.7 & 5.4 & 92.4 \\
         0.1& \textbf{35.1} & 0.0 & 10.8 & 85.8 \\
         0.2& \textbf{42.9} & 5.4 & 7.9  & 89.5 \\
         0.3& \textbf{54.6} & 0.9 & 8.9  & 88.8 \\
         0.4& \textbf{60.7} & 0.9 & 12.2 & 85.9 \\
         0.5& \textbf{68.0} & 50.7 & 14.3 & 83.1\\
    \end{tabular}
    \label{tab:execution-time}
\end{table}

%\begin{table}
%    \centering
%    \caption{Performance comparison of PCGRL with hill climbing approaches for optimizing different balancing values $b$. All values are expressed as percentages.}
%    \begin{tabular}{ll|cccccc}
%        &&   \multicolumn{6}{c}{$b$} \\
%         & &  0.0 & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\  \hline
%         & Initial $=b$         & 8.6  & 7.2  & 6.4  & 11.4 & 12.0 & 15.6 \\ \hline
%        PCGRL & \multicolumn{1}{|l|}{Balanced to $b$ }    & 36.1 & 35.1 & 42.9 & 54.6 & 60.7 & 68.0 \\
%        S-wide & \multicolumn{1}{|l|}{Improved to $b$} & 71.1 & 73.5 & 76.3 & 77.9 & 81.4 & 88.9 \\
%         & \multicolumn{1}{|l|}{Baseline} & - & - & - & - & - & 48.1\\ \hline
%       Hill -  & \multicolumn{1}{|l|}{S-narrow} & 30.7 & 0.0 & 5.4 & 0.9 & 0.9 & 50.7  \\
%       Climbing  & \multicolumn{1}{|l|}{narrow}   & - & - & - & - & - & - \\
%    \end{tabular}
%    \label{tab:execution-time}
%\end{table}



\subsection{Evaluation of the asymmetries of the generated levels}
\label{sec:asymmetries}
The motivation behind this work includes the creation of asymmetric game levels to enhance diversity for competitive play. To evaluate this goal, we assess all generated levels across all models outlined in Section~\ref{sec:unbalancing} to evaluate their symmetrical properties.

The symmetry of an $n \times n$ matrix $M$ can be evaluated using the Frobenius norm [X] which computes the sum of the absolute differences of matrix elements. As we are dealing with non-numerical tile representations, however, this is not applicable.
To overcome this limitation, we measure the proportion of unequal tiles along the horizontal, vertical, diagonal, and counter-diagonal symmetry axes relative to the size of the matrix. This concept is expressed by Eq.~\ref{eq:symmetry}, which is defined in $[0,1]$. A value of 1 denotes a symmetrical level, while 0 signifies an asymmetrical one. The matrix $M'$ is derived from $M$ according to the selection of the axis for symmetry evaluation process.

\begin{equation}
\label{eq:symmetry}
sym(M, M') = \left( \sum_{i=1}^{n} h(M_i, M'_i) \right) \cdot \frac{1}{n^2}
\end{equation}

The auxiliary function $h$ returns 1 if $M_i = M'_i$, otherwise 0. $M_{rot}$ denotes $M$ rotated counterclockwise by 90 or 180 degrees respectively, $M^T$ the transposed matrix of $M$. To compute the symmetry score for the diagonal axis we compute $sym(M, M^T)$, for the counter-diagonal $sym(M, (M^T)_{rot180})$, the vertical $sym(M, (M_{rot90})^T)$, and the horizontal $sym(M, (M^T)_{rot90})$. The mean, standard deviation, minimal, and maximum values are presented for the four symmetry axes in Table~\ref{tab:symmetries}.

\begin{table}
    \centering
    \caption{Overview of symmetry scores for generated levels across four axes using Eq.~\ref{eq:symmetry}. A value of 1 indicates full symmetry along an axis, 0 full asymmetry.}
    \begin{tabular}{c|c|c|c|c}
           &  \textbf{diagonal}&  \textbf{counter-diagonal} & \textbf{vertical} & \textbf{horizontal} \\ \hline
         Mean &  0.428 &  0.432 &  0.316 & 0.313 \\
         Std. &  0.099 &  0.097 &  0.107 & 0.106 \\
         Min. &  0.167 &  0.167 &  0.0   & 0.0\\
         Max. &  0.778 &  0.778 &  0.722 & 0.667\\
    \end{tabular}
    \label{tab:symmetries}
\end{table}

The results show none of the generated levels for any model are symmetrical. 

\section{Discussion and limitations}
\label{sec:discussion}
% In this work, we proposed a method for automated level balancing with RL. We showed our method using swap-based representations performs better within less training steps compared to the original PCGRL.
Our experiments showed promising results within fewer training steps compared to the original PCGRL while being more robust to ensure playability. There are, however, several things that need to be discussed.

The reward of the balancing agent represents the balancing state of multiple simulations on the current level state. By design, this is done with the use of the information of which player won per simulation pass. Using game specific information such as e.g., the health state of players inside the reward function potentially might improve the results. This is, however, not desired since including domain specific information creates dependencies on the distinct game. In this case, a special reward function must be developed for each game. Furthermore, including too much or the wrong information could bias the reward resulting in poor performance or unwanted behavior of the model. \hl{Consequently}, the model would not learn what \emph{really} influences balancing, or it might exploit unforeseen loopholes.


Splitting up the level generation and balancing process into separated units yielded much better results than doing it in the same step as in the original PCGRL. 
The plain PCGRL might be able to achieve comparable results when trained significantly longer, however, the here proposed architecture converges faster in less updates of the policy. This gives evidence that our architecture is more efficient by subdividing the problem into two simpler problems. In combination with the swapping representations, the balancing process can fully focus on balancing. We compared three adapted representations from the original PCGRL and evaluated them regarding performance. All of them can improve the balancing state, whereas swap-turtle yielded slightly worse results than the other two. Thus, swap-narrow, and swap-wide perform comparably, we recommend using the narrow representation when faster training and generation is required. It is, furthermore, independent from the grid size. If the focus is on performance\hl{,} we recommend using the swap-wide representation.
%\hl{Through matrix comparisons, we determined a content diversity of 100\% of the generated and balanced levels. This is a solution at the value layer, however, not at the semantic one. There may be levels that are semantically the same e.g., if a few tiles are different, which has no influence on the game. This process cannot be easily automated. A manual examination of a random subset of 50, no semantically identical levels could be found.}

Since we showed that the model improves a level's balancing significantly, it is possible to draw conclusions about which tile types have most impact on balancing regarding their swap-frequencies.
For this domain, the swapping of resource tiles (e.g., forest) with blocking elements (stone) had the greatest impact. Swapping players' spawn position was not a favored action. We assume that this is due to the small number of available types of this type (only two) compared to resource tiles and therefore the model had less experience in learning these swaps appropriately.

By simulating the game $n$-times with player agents the balancing state is evaluated. This metric is of course dependent on exactly these types of players. In online gaming, the pairing of players of the same skills is often ensured through matchmaking algorithms~\cite{alman_theoretical_2017} that utilize the Elo-rating system~\cite{elo_rating_1978}.
For players with e.g., different skill or type the balancing would be different. That is a limitation, however, being also an advantage. By using different types of player agents, the game level could be balanced to compensate skill differences of the players by solely adjusting the level not the players themselves. This is of high interest when balancing levels for different player types such as a mage and a fighter. It can be applied in e.g., role play games where gear levels are an indicator of the character strength. So, players can use their long-farmed equipment in a competitive setting and the game could be balanced through the environment only. In future research, our work is to be extended towards this. The controllable content generators~\cite{earle_learning_2021} might be an applicable solution in that context.

\hl{One challenge with the proposed architecture involves the computational effort during model training. This is particularly due to the simulation step required for reward calculation, as with every swap made by the agent, a simulation step is initiated.
RL learns throughout training trajectories, offering an optimized approach to reduce unnecessary swaps and therefore computational effort at inference.
%The reason why RL is an appropriate method to apply here is as it learns during training. 
We contrasted our method with a hill climbing approach which relies heavily on randomness and necessitates restarting from scratch with each new iteration. %, leading to unnecessary simulation steps that may e.g., have no effect on the balancing state. Conversely, RL learns throughout training full trajectories, offering a more optimized approach.
The comparison demonstrated PCGRL's superior execution speed and greater consistency in execution times across all models.}
%In contrast, e.g., an evolutionary approach would need unnecessary steps of evaluating its fitness since it starts over again each time from scratch.


In addition, we figured out that the reward is mostly sparse in training. That indicates, only a small sub sample of the action space are actions which influence the balancing. Especially in the beginning of the training, this must be learnt by the model first.
In order to speed up the training process, we are considering methods that reduce the computational effort. This would also be of great interest for the application in more complex environments.
One solution might be to reward the agent after several time steps only or even use sparse rewards. Despite the learning process would then be harder for the agent, simulation steps for the reward are omitted. Thus, the training process is sped up and the agent can explore faster.
Another approach could be the usage of a surrogate reward model to predict a level's balancing state. This would speed up training a lot, however, the model's accuracy must be high enough to give appropriate rewards to ensure a correct training. Lowering the reward calculation costs thereby improves the feasibility of an evolutionary algorithm. Investigating the swap-based representation pattern incorporated into the crossovers or mutations of an evolutionary algorithm represents an interesting target for future research.

\subsection{Discussion on the application of fairness metrics for game balancing}
We've automated the decision-making process of how balanced a game is, based on a function inspired from the Statistical Parity metric~\cite{dwork_fairness_2012}.
This metric is commonly used in the fair machine learning community for e.g., to measure how fair automated decision-making systems based on machine learning are~\cite{makhlouf_applicability_2021}. With this section, we want to open the discussion on how fairness metrics can be applied to game balancing in general. At this point, it is important to mention, that the concept of fairness is a social and ethical concept and not a statistical~\cite{chouldechova_fair_2017}. Games are, however, designed to be played by humans. Therefore, social and ethical considerations should be considered when applying an automated balancing process, particularly in a competitive environment with multiple players.

\paragraph{An acceptable range of win rates} So far, we only considered the balancing proceeding for a level as success if the metric corresponded exactly to the predefined balancing goal (e.g., $b=0.5$). An exact measuring of a certain value through sampling is, however, in many cases not achievable. Although we have examined how often we should sample to find a balance between the number of simulation runs and minimizing uncertainty for the estimation of the actual game balance, there is still a residual uncertainty. This is also a problem that often arises when collecting data about the real world such as surveys etc. To address this issue, a solution is the introduction of a bias and define the optimal value not as a single value, but as a range. The \emph{Disparate Impact} metric~\cite{feldman_certifying_2015,saleiro_aequitas_2018} expresses fairness with the ratio of a predicted outcome of two groups. The fairest ratio here would be represented by a value of 1. A commonly used range for this metric to consider an outcome as fair is~$>=0.8$ as stated in~\cite{saleiro_aequitas_2018}. That being said, applied to game balancing values in a range to the desired value can be considered as balanced. For this work, we could define a balanced game state as: $1-(w_{p1t} - w_{p2t}) \ge 0.8$. Introducing this bias would increase the range of levels considered balanced, resulting in an even better proportion of balanced levels in our method. Since this bias has a strong influence on that proportion, it should be adapted to the game domain regarding the residual uncertainty when transferred to game balancing.



\section{Conclusion and Future Work}
\label{sec:conclusion}
In this paper, we proposed a new method to balance tile-based game levels with reinforcement learning (RL).
Therefore, we introduced a novel swap-based representation family for the PCGRL framework, where the RL agent swaps the locations of tiles in a given level.
Our architecture benefits from separating the level generation and balancing process into two subsequent processes. The latter can therefore be considered as a task for fine-tuning existing content.
In this extended article we discussed the application of existing fairness metrics to game balancing and thus derived the reward function for the RL from the Statistical Parity metric, in order to automatically measure the balancing state of a level.
%and include information from simulated game runs.
Furthermore, we improved the results from the conference paper on level balancing to a proportion of balanced levels of 68\% and the proportion of improvements to 88.9\%. Compared to the original PCGRL method (30.4\%) on generated levels of the NMMO environment, our approach is easier to learn and significantly improves the results.

In addition, our approach is generalized\hl{,} and we have shown how one can also generate levels with a specific balance in order to generate unbalanced levels that favor a specific player. This opens new perspectives to create levels when e.g., adults play vs. children or for players with different gear levels.
Finally, by analyzing which tiles are swapped frequently, information can be inferred which tile types influence the balancing most. This provides game developers with additional empirical evidence about how the game system itself actually behaves.

For future work, we want to test our method with increased player sizes. Additionally, the balancing for players of different types like e.g., a mage versus an archer by only altering the game level is of interest. Moreover, we think that this method is applicable not only to games, but also to other domains as well. In subsequent research we are interested in the application to city planning for fair infrastructure distribution.

\section*{Acknowledgments}
We thank Christoph Kern, Frederic Gerdon, Jakob Kappenberger, and Lea Cohausz for their feedback and discussions on fairness metrics. We would also like to thank Patrick Takenaka for further feedback and comments.

==> content/content_revision1.tex <==
\section{Introduction}
 
The design of levels is a key concept when creating games. To keep players engaged, the balance between a challenging and enjoyable experience must be found. This is generally not an easy task, as it also depends on the skill and experience of the players~\cite{schreiber_game_2021}.
Furthermore, game levels for competitive multi-player games must be designed to be balanced towards equal initial win chances for all players. Imbalanced games will result in boredom or frustration and players will quit playing~\cite{andrade_dynamic_2006,becker_what_2020}.

To ensure balancing through the level design, game designers often rely on almost (point) symmetric map architectures. This can be seen in popular competitive esports titles such as League of Legends, DotA~2 or Starcraft~2, but also in other competitive tile-based games such as Advance Wars or Bomberman.
\hl{In addition to symmetrical levels, alternative approaches are also possible.} Non-symmetrical levels offer more diversity and can create new ways for playful creativity to be entertaining and challenging.

For this work we frame the balancing task for levels as a procedural content generation (PCG) task. In previous works, several approaches have been proposed using (PCG) for level balancing, such as search-based approaches~\cite{togelius_search-based_2011,sorochan_generating_2022}, evolutionary algorithms~\cite{morosan_automated_2017,lanzi_evolving_2014,lara-cabrera_balance_2014,karavolos_using_2018,mesentier_silva_evolving_2019} or graph grammars~\cite{kowalski_strategic_2018}.
In this work, we introduce the balancing of tile-based levels with reinforcement learning (RL). Once a RL model is trained, it can generate levels fast and is less dependent on randomness compared to evolutionary methods. We apply RL for balancing by designing a reward function based on multiple simulation runs using scripted agents. While this approach becomes computationally intensive due to the simulations for each reward calculation, RL's advantage over evolutionary algorithms lies in learning during training. This reduces the need for unnecessary simulations in the inference step, unlike evolutionary algorithms that start anew each time.
In addition, we develop our method to not be dependent on a single domain, as is the case with graph grammars or search-based approaches.

\begin{figure}
     \centering
        \includegraphics[width=2.8in]{content/images/res_water2.png}
    % \includegraphics[width=2.8in]{content/images/example1.png}
    \caption{
In our game environment, two players must forage for resources like food (dark green) and water (blue) to survive longest. By swapping the highlighted tiles (red), the trained model reached a more balanced game in simulated game runs. 
}
     \label{fig:gen-level1}
\end{figure}

Therefore, we use the procedural content generation via reinforcement learning framework (PCGRL)~\cite{khalifa_pcgrl_2020} which recently has been introduced for the generation of tile-based levels. Together with newly introduced swapping representations, our method can be viewed as a fine-tuning task to optimize a generated level towards a certain balance.
Our method is evaluated on the openly available Neural Massively Multiplayer Online (NMMO) environment~\cite{suarez_neural_2019} which has been designed for competitive multi-player research. We frame the problem as a resource gathering and survival game. Figure~\ref{fig:gen-level1} shows an example of how our method balanced a generated level (left) by swapping highlighted tiles (right). The code used in this research is available \hl{on} Github\footnote{https://github.com/FlorianRupp/pcgrl-simulation-driven-balancing}.

Our contributions are:
\begin{itemize}
    \item A domain independent architecture for learning the automated altering of game levels towards a specified balancing with RL. 
    \item A novel swap-based representation pattern to frame the problem as Markov decision process.
    \item An experimental study to evaluate the proposed architecture compared to the original PCGRL method.
\end{itemize}

This paper is an extended version of the conference paper~\cite{rupp_balancing_2023}. We provide improved results, a detailed discussion on how existing fairness metrics can be transferred to game balancing, and a study of how this can be used for any balancing and not only equal balancing. Therefore, we revise the reward function and explain its derivation from the Statistical Parity metric~\cite{dwork_fairness_2012}.

The structure of this paper is as follows: We give a brief overview of related work~(\ref{sec:related-work}) and the background~(\ref{sec:background}). In Section~\ref{sec:method} the method is described and the implementation details in~\ref{sec:details} subsequently. Experiments and results are presented in~\ref{sec:experiments}, followed by an extended study on the generalized approach of an arbitrary balancing in~\ref{sec:extensions}. The discussion is in Section~\ref{sec:discussion}, the conclusion in~\ref{sec:conclusion}.

\section{Related work}
\label{sec:related-work}
% game balancing
For multiplayer \emph{game balancing}, several methods have been proposed in the past. One approach is the balancing through the configuration of game entities such as characters, weapons or items~\cite{schreiber_game_2021}. To do this, the games industry uses pipelines to extract data-driven insights from played games to adjust the balancing in a regular schedule\footnote{https://www.leagueoflegends.com/en-gb/news/dev/dev-balance-framework-update/}.

\hl{Evolutionary algorithms are further widely applied for game balancing.
Morosan et al. balance a real time strategy game (RTS)}~\cite{morosan_automated_2017} \hl{and Sorochan et al. generate new and balanced units for an RTS game}~\cite{sorochan_generating_2022}.
\hl{De Mesentier Silva optimize cards for the game Hearthstone}~\cite{mesentier_silva_evolving_2019} \hl{to balance its metagame.
Another approach trains models with data from played games to replicate human behavior for automated balancing of entities}~\cite{pfau_dungeons_2020}.

%A different method, especially in online games, are matchmaking algorithms~\cite{alman_theoretical_2017}. These methods assign which players play against each other or are in the same team and contributes to balancing by ensuring that the players' skill in a match is at a comparable level. Multiple works on this exist, however, many are based on a form of the Elo rating system~\cite{elo_rating_1978} used by the World Chess Foundation where a player's skill can be expressed by a single number. To integrate more information into the process and also improve player satisfaction, match making in~\cite{deng_globally_2021} is framed as an MDP to apply RL in a sequential task.  

The balancing of a level is furthermore influenced by its design. That refers to e.g., the position where game entities are located in relation to players' initial spawn position. As aforementioned, it is ensured with (point) symmetric map architectures in many games.
Contrary to the intended balancing the perception of players may differ. A survey concluded that a prevailing opinion among high experienced players is that only symmetrical levels can actually be balanced~\cite{togelius_controllable_2013}.

To automatically construct balanced levels with PCG, work has been introduced using evolutionary algorithms~\cite{lanzi_evolving_2014,lara-cabrera_balance_2014}. In contrast to this work, the fitness for balancing is evaluated rule based with heuristics or metrics. These metrics are either handcrafted or rely on a data-driven method using played games. In~\cite{karavolos_using_2018} this is extended with a convolutional neural network to predict game related information which are then used in the fitness function of an evolutionary algorithm to produce balanced levels. A different approach is the usage of graph grammars~\cite{kowalski_strategic_2018}. The balancing here is constructed by the rule-based placing of strategic game entities, which is, however, very dependent on the domain.

%In \cite{delaurentis_toward_2021} is a framework proposed to predict the balancing state based on played games with bots to balance a game.

% PCG
In this work, we focus on \emph{procedural content generation} for level generation, but the term PCG is also used in other applications such as the generation of game economies~\cite{rogers_using_2023}, rules~\cite{cook_mechanic_2013} or narratives~\cite{alvarez_tropetwist_2022}. PCG methods span over from dedicated algorithms~\cite{mojang_mincraft_2011}, search based methods~\cite{togelius_search-based_2011,lanzi_evolving_2014,lara-cabrera_balance_2014} up to the use of machine learning~\cite{summerville_procedural_2018} and deep learning~\cite{liu_deep_2021,giacomello_doom_2018,awiszus_toad-gan_2020,sudhakaran_prompt-guided_2023}. 
Once trained, machine learning-based methods can quickly generate content as needed, but they rely on having game levels already available from which a model can be learned. Therefore, when creating new games, these methods are usually not applicable efficiently.

In the games community, RL has been widely applied to \emph{play} games~\cite{silver_general_2018, vinyals_grandmaster_2019}, but recently, it has also been used for PCG~\cite{khalifa_pcgrl_2020,bontrager_learning_2021,gisslen_adversarial_2021,zakaria_procedural_2022}.
\hl{The framework we use and extend in this work is PCGRL}~\cite{khalifa_pcgrl_2020},\hl{ utilizing RL for PCG tasks (cf. Section}~\ref{sec:pcgrl}).
\hl{Zakaria et al. compare different deep learning-based PCG approaches for the puzzle game Sokoban, with \mbox{PCGRL} showing superior quality}~\cite{zakaria_procedural_2022}.
There are already quite a number of methods which adapted the PCGRL method. In \cite{earle_learning_2021} controllable content generators were introduced, where users control the generated content with additional constraints, such as e.g., the number of players.  
We do, however, not compare our method with it, as our objective is a balanced level only.
Other approaches use evolutionary strategies on top of the PCGRL framework to achieve more content diversity~\cite{khalifa_mutation_2022} or adapted the method for 3D environments \cite{jiang_learning_2022-4}.


\section{Background}
\label{sec:background}
\subsection{The PCGRL framework}
\label{sec:pcgrl}
In this work, we use the PCGRL \cite{khalifa_pcgrl_2020} framework for level balancing.
In PCGRL, PCG is formulated as a sequential decision-making task to maximize a given reward function, where semantic constraints can be expressed and thus, no training data is needed. To apply RL, the PCG problem is framed as a Markov decision process (MDP).

Therefore, PCGRL introduces three different MDP representations for level generation. 
We will introduce three new swap representations based on the existing representations. Later we argument that they are a better fit to alter game levels to improve e.g., the balancing state. The original representations in PCGRL are: 

\paragraph{Narrow} This representation randomly selects a tile in the grid and the agent only needs to decide what type of tile should be placed on the selected position. This has a small action space since it only consists of the different types of tiles. 

\paragraph{Turtle} The \emph{turtle} representation allows the agent to move on the map and then to decide what type of tile to put on the current position. The advantage to the narrow representation is that the agent is not restricted to the randomly assigned position and therefore can learn where to move next.

\paragraph{Wide} In the \emph{wide} representation the agent is given full control of the level generation process as the agent can decide which tile of the whole grid should be changed. This increases the action space greatly thus every position of the grid multiplied by the number of tiles represents an action. This is the most human-like representation as the agent can change everything directly according to a plan it has constructed.

\subsection{The Neural MMO Environment}
\label{sec:nmmo}
As basis for our experiments, we use the NMMO environment~\cite{suarez_neural_2019}. The NMMO environment is a Massively Multiplayer Online Battle Royal inspired multi-agent RL environment for research.
It simulates a tile based virtual world where agents must forage for resources to survive and be prepared for fights with other agents. All actions of the agents are processed simultaneously per time step. The agent which survives the longest wins the game.
The agent's state is represented by its position as well as its current health, food, and water level.


In this paper, we focus on the balancing in the PCG process of the game map. To apply and evaluate our method, we simplify the win condition and frame the game as a forage survival game. Therefore, we disable the combat system and limit map tiles to the types of grass, forest, stone, and water. The agent cannot move on stone nor water tiles. Forest and water are resources the agent can gather. A detailed overview of the tiles and their behaviors is given in Figure~\ref{fig:tile-descr}. When moving on a forest tile, it is consumed automatically as food and refills the agent's food indicator. In the process the forest tile changes to the state \emph{scrub}. Scrub tiles cannot be consumed, however, there is a probability of 2.5\% per time step to respawn and transit back to the forest state.
To refill the agent's water indicator it must simply step on an adjacent tile. Water tiles are not depleted. If one of both resource indicators are empty the agent loses a fixed amount of health per step. If the agent's health indicator drops to zero, the agent dies. An agent can restore health having water and food indicators over 50\%. 

\begin{figure}
     \centering
     \includegraphics[width=0.7\linewidth]{content/images/tiles.png}
     \caption{Description of the NMMO tiles.}
     \label{fig:tile-descr}
\end{figure}

For this research we frame the win condition equally for both agents. The agent which completes one of two goals first wins:
\begin{itemize}
    \item Collect five food resources.
    \item Last agent standing: Not starved nor died of thirst.
\end{itemize}

In this introductory research, we fix the map size to a grid of 6x6 tiles and two players to speed up the experiments and to keep the results interpretable by human evaluators. Furthermore, the smaller grid size limits the available space and resources which reinforces the competitive race of the agents. This competitive race is to be balanced in this paper.


\section{Method}
\label{sec:method}
\subsection{Balancing architecture}
\label{sec:architecture}

\begin{figure*}
  \centering
  \includegraphics[width=0.9\linewidth]{content/images/balancing-architecture.png}
  \caption{Description of the balancing architecture. It is separated into three units: A level generator, a level balancing agent and a level playing simulation. In the latter, the game is simulated by playing it $n$-times with player agents. The reward $r_t$ for training the balancing agent is calculated out of the balancing states $b_t$ and $b_{t-1}$ from the simulations.}
  \label{fig:architecture}
\end{figure*}

This paper proposes an architecture to balance tile-based levels with RL. The idea is to reward a PCGRL agent for only altering a given playable level towards a balanced level.
A balanced level is a level where all player agents with the same skill have the same win rate.
\hl{We only focus on game balance through level design, which excludes balancing a sequence of levels or different play styles for instance.}
The architecture is depicted in Figure~\ref{fig:architecture}. It is separated into three parts: a level generator, a balancing agent and a playing simulation. 

% short descr of gen agent
The level generator constructs a playable level from random noise which is then fed to the balancing agent. \hl{In this work} we use PCGRL for the generator, however, other PCG methods will serve at this point comparable. The generator is trained separately before training the balancing agent.

% short descr of balancing agent
The core idea to balance the level is not to generate a new level but to modify the given level accordingly to fulfill the balancing constraint.
Each time step the balancing agent can decide to swap the positions of two selected tiles. If a swap (Section \ref{sec:swap}) was made, the level is played $n$-times in a simulation by player agents. Subsequently, the balancing agent is rewarded based on how this action influenced the balancing state in simulations (Section \ref{sec:reward}). This is inspired from the idea of simulation-based fitness functions in~\cite{togelius_search-based_2011}.

More details are given in the implementation details~(Section~\ref{sec:details}).


\subsection{Swap-based representation pattern}
\label{sec:swap}
To formulate the problem of PCG with RL as MDP three representations have been introduced in \cite{khalifa_pcgrl_2020}. In all of them the agent can decide to replace a tile at a distinct position. This method, however, may result in unplayable levels at a time step. Furthermore, to move the position of e.g., a player tile somewhere else, the agent would need to remove the player tile first before creating it at a different position. In this time step the level would not be playable for the player agents and thus, no reward could be computed in the simulation step. Additionally, the agent would get a negative reward first due to the number of players is now invalid. The subsequent creation at a different position under the previously given negative reward is hard to learn for RL agents.

For this reason, we introduce a swapping-based representation pattern. In these representations the agent can decide to swap the positions of two tiles per time step.
Not adding or removing tiles entirely is a more robust approach to ensure level playability.

There might be, however, game domains where multiple tiles have a semantic connection e.g., multiple river tiles construct a river. Swapping these tiles around can break playability. \hl{Therefore}, we suggest in the balancing step to feed unplayable levels back to the generator to fix it again.
This repair is similar to the level fixing seen in~\cite{siper_path_2022}\hl{, but it would also involve an additional increase in computational effort.}

In this work we demonstrate the power of swapping with a simpler domain where no semantic relations of multiple tiles exist. In addition, swapping tiles ensures that the old level isn't simply generated from scratch since that's the job of the level generator.
Swapping two tiles of the same type has no effect on balancing. Thus, we prevent these swaps to reduce computational intensity. In these cases, the agent is rewarded with 0.
Therefore, we extend the narrow, turtle and wide representations~\cite{khalifa_pcgrl_2020} with a swapping mechanism:

\paragraph{Swap-Narrow} As in PCGRL the agent observes the tiles in the environment one-hot encoded. At each time step two random tile positions are presented to the agent, and it can decide to swap the tiles or not. The agent's little position control results in in a very small action space $A$ with only two actions: swap or do not swap. $A$ is therefore $A=[2]$.
\paragraph{Swap-Turtle} Starting at two random positions the agent can decide to swap the tiles at the current positions in each time step. If no change is made it can decide to which adjacent tile to move next. \hl{As in the original PCGRL, staying in one position and not changing a tile is not an option.} The observations are in a one-hot encoded format as well. $A$ is therefore $A=[4,4,2]$ which results in 32 possible actions.
\paragraph{Swap-Wide} In this representation the agent sees the whole level and can freely determine the tile positions and whether to swap it. The observations are provided one-hot encoded. It can be interpreted as looking at the whole level and then decide what to move where. A drawback here is the large action space since it scales twice with the grid width $w$ and height $h$. $A$ is therefore $A=[w,h,w,h,2]$. In the case of a square grid shape as in this work with a size of 6, $A$ has 2592 possible actions.

\subsection{Reward design}
\label{sec:reward}
For the successful training of a RL agent, the reward function is crucial. Heuristic approaches for the evaluation of balancing have been introduced in~\cite{lanzi_evolving_2014,lara-cabrera_balance_2014}. These approaches, however, include domain specific information and are thus not transferable. To address this shortcoming, we propose the use of a more generic, game domain independent reward function only relying on how often each player wins. In addition, we require the game to have at least one winner at its end. Since draws also provide information about the balancing state, our reward function must handle this as well.

To measure the balancing appropriately, we are inspired by fairness metrics from the fair machine learning community. A survey of common metrics used in that field is provided in~\cite{makhlouf_applicability_2021}. The Statistical Parity metric~\cite{dwork_fairness_2012} is one of them and often used to measure fairness between two groups. The fairness for two groups $G=1$ and $G=2$ is considered as fair if the conditional probability of the same outcome $\hat{Y}$ for both groups is the same, as seen in Eq.~\ref{eq:stat-parity}. 

\begin{equation}
\label{eq:stat-parity}
P(\hat{Y}\,|\,G = 1) = P(\hat{Y}\,|\,G = 2)
\end{equation}

In this work, we transfer this definition of fairness to the domain of game balancing. 
In the context of the Statistical Parity, the two groups represent the two players and we want to optimize their win rates.
%, cf. $P(win \,|\, player = 1) = P(win \,|\, player = 2)$. 
However, the direct use of Eq.~\ref{eq:stat-parity} is not applicable to RL since it requires a function that rewards the agent with positive or negative incentives per time step $t$. In addition, an intermediate reward design which compares $t$ to $t-1$ has shown good results in PCGRL.
First, we therefore define the win rate $w_{p_it}$ per player $p_i$:
\begin{equation}
\label{eq:bt}
w_{p_it} = P(w_t\,|\,p = i)
\end{equation}
$w_{p_it}$ is then inferred from the data from the $n$-runs of the player agent simulations per step. This could be viewed as a sampling from the actual win rate distribution (cf. Section~\ref{sec:simulation} and Fig.~\ref{img:balancing}).
Second, in this extended paper we additionally want to make the reward design configurable to a certain balancing state $b$ and thus rewrite the balancing calculation $b_t$ as:

\begin{equation}
\label{eq:b}
b_t = |\, w_{p_1t} - b \,|
\end{equation}

%The balancing state $b_t$ is the absolute value of the deviation of a player from $b$.
Due to the use of the absolute value, $w_{p_it}$ of both players could be used in Eq.~\ref{eq:b} as their values describe probabilities which sum up to 1.
%We design the reward function to reward the agent for improving the balancing state $b_t$ in time step $t$ in comparison to $b_{t-1}$.
$b_t$ is defined in $[0,1]$ as well where 0 indicates $b_t$ corresponds exactly to $b$; 1 indicates the maximal deviation from $b$. In the example where an exact balance between both players is desired ($b=0.5$), $b_t=1$ indicates one distinct player wins every game.
\hl{With $b_t$ in this range, there is flexibility to configure toward which player the game should be balanced to.}
Finally, the reward $r_t$ is: 
\begin{equation}
\label{eq:reward}
r_t = b_{t-1} - b_t  + \alpha
\end{equation}

To additionally reward the agent, a reward $\alpha$ is given if $b_t$ is exactly $b$. Otherwise, $\alpha$ is 0. \hl{If $\alpha>0$ the episode always ends as $b_t=b$.}
As a result, the reward will be positive if the agent improves the balancing state, negative otherwise. For no impact on the balancing state the agent receives no reward (value 0). Applying this reward design, the RL agent is gradually incentivized to reduce the absolute difference from current balancing state to the intended one.


\section{Implementation details}
\label{sec:details}
\subsection{Level generator}
\label{sec:gen}

The task of this unit is to generate playable levels for balancing. In this work, the generator is a model trained using the PCGRL framework.

The reward for the training process is designed to reward the agent to
\begin{itemize}
    \item have exactly two players and
    \item create a valid path between both players.
\end{itemize}

To guarantee the direct competition, the latter constraint ensures that both players have access to the same area of the game level. Additionally, this prevents single players being locked within stone walls.

The NMMO environment uses by default PCG to generate random levels, however, the players' spawn positions are randomly determined when the game starts. Nonetheless, the spawn positions are crucial for balancing and thus, should be possible to be aware of and to influence by the balancing agent. For this reason, a player tile is integrated in the level generation process representing the positions.

If a valid path between both players exists the agent receives a positive reward, a negative otherwise. Additionally, each step the agent is rewarded with the difference of players there are and should be (similar to \cite{khalifa_pcgrl_2020}). We achieve the best results using the \emph{wide} representation. An episode ends when both constraints are met, or the agent exceeds a fixed number of permitted steps or changes.

After training, the model can produce levels satisfying the given constraints in 98,7\% levels out of an evaluation sample of 5000. \hl{The generated levels achieve a maximum diversity at 100\%, so no two levels are completely identical.} An example of a generated level is shown in Figure~\ref{fig:gen-level1}~(left) and a tile legend is given in Figure~\ref{fig:tile-descr}.

The yielded levels are then \hl{passed on} to the balancing agent. Level generation at this step is done until the agent produced a valid level fulfilling the constraints to ensure the balancing agent receives playable levels only.

%\begin{figure}[!t]
%  \centering
%  \label{img:genagent}
%  \includegraphics[width=2.5in]{content/images/pcgrl_map.png}
%  \caption{A playable, not yet balanced game level for the NMMO environment generated with PCGRL. Exactly two players exist which are connected. The colored tiles represent the NMMO tiles: blue=water, grey=stone, light green=grass and, dark green=forest. Additionally the spawn positions of the players are represented with the face icon.}
%\end{figure}


\subsection{Balancing agent}
\label{sec:balancing}
The balancing agent is the core component of the architecture in Figure \ref{fig:architecture}. We model the agent as PCGRL agent which can decide to alter a previously generated game level per time step. To support this process, we use swapping representations.
The reward is calculated out of the results of a simulation of the balancing state (Section \ref{sec:reward}).

The observation is the current level one-hot encoded. In detail, this depends on the chosen representation. As RL algorithm, we apply PPO (proximal policy optimization)~\cite{schulman_proximal_2017}.
An episode ends when the level is either balanced, or a fixed number of steps or changes is exceeded. \hl{In PCGRL, the number of changes allowed is determined relative to the grid size (cf. change percentage). As in the original PCGRL we use a change percentage of 20\%. We set the value for the number of allowed steps within an episode to 100.}

\subsection{Player simulation}
\label{sec:simulation}
To calculate $b_t$ for the reward (Section~\ref{sec:balancing}) we run a simulation $n$-times of player agents playing the game.
The player agents can be any solution which can simulate a player's behavior at a required quality. In this work we use the scripted \emph{Forage}-agent for the NMMO environment which is publicly available\footnote{https://github.com/NeuralMMO/baselines}. The usage of scripted agents provides the benefit of a deterministic behavior at any time step. If the agent's water or food indicator drops below a certain threshold it looks for the next available resource of that type to refill it.
At this point, however, the application of trained agents with e.g., RL, different skilled or types of agents is feasible as well. See the discussion~(Section~\ref{sec:discussion}) for further information.

Despite running the simulation with the same player agents, winners may differ each pass. This is because of probabilistic mechanics making games interesting such as rolling dices or the respawn of resources at a certain probability. A player may win with luck, but when playing many times, skill should make the difference. The question is then, how often must a simulation be run to minimize the noise of probability? \hl{Due to simulating} is computationally intensive, it is of interest to find the number of minimal runs where win rates vary at an acceptable level.

We approach this by investigating how much the win rates $w_n$ of a specific number of simulations $n$ differ on average from $n-2$. Only even values for $n$ are applicable since otherwise a balanced game is not possible. Therefore, we run the simulation on a sample of size $s=500$ levels up to a number of \hl{$N=30$} times and compare how win rates for $n$ fluctuate on average in comparison to $n-2$. The average deviation~$\mu_n$ of a distinct $n$ is expressed with: $\mu_n = \frac{1}{s} \sum^{N}_{n=0} | w_n - w_{n-2} |$ and its course is depicted in Figure~\ref{img:balancing}. In addition, the standard deviation is given with $\sigma$ and $2\sigma$. It is clear that the larger $n$ is, the smaller $\mu_n$ is. To determine an appropriate $n$ we set the threshold: $\mu_n + \sigma < 0.05$. For this game with the configured number of players, this applies to $n \ge 14$. Therefore, we use $n=14$ in this work.


\begin{figure}[!t]
  \centering
  \includegraphics[width=3.1in]{content/images/balancing_metric.png}
  \caption{How many times $n$ should we run the simulation to approximate the balancing state? We figure that out by calculating the mean deviation $\mu_n$ of win rates from $n-2$ to $n$ for the investigation of fluctuations in win rates.}
  \label{img:balancing}
\end{figure}

This method can be used to determine $n$ for any domain.


\section{Experiments and Results}
\label{sec:experiments}

We evaluate our architecture in several steps: First of all, we sample a fixed data set of levels to use for direct comparison with the generator. Then we compare the balancing performances of the three introduced representations with the original PCGRL method as a baseline~(\ref{sec:eval-swap}). To generate balanced levels with the original PCGRL method, we integrated the balancing constraint into the reward function.

Subsequently, we investigate on the levels the models created~(\ref{sec:gen-levels}) and examine which tiles the models swapped in the level altering process~(\ref{sec:impact}). The latter can provide insights about which tiles actually influences the balancing.

\subsection{Performance overall}
\label{sec:eval-swap}
We compare the performance of the swap representations among themselves and in contrast to the original PCGRL as baseline\footnote{Only the narrow representation is shown here; the other two yield similar results.}. For direct comparison all models have been trained the same amount of 200k training steps resulting in 970 updates of the policy.

For the evaluation we create a data set of 1000 levels with \hl{our PCGRL} generator. This data set is then used for all four models for evaluation.
First of all, we investigate on the distribution of initial balancing states of the levels in the data set (see Figure~\ref{fig:init-balancing}). Important to mention here is the non-equal distribution. Except the states 0 and 1 the levels seem to be normal distributed around the state of 0.5, indicating both players won equally often. A share of 13.6\% of levels is initially balanced. However, peaks towards maximally unbalanced levels at the outer edges of the distribution can be observed. Maximally unbalanced levels make up 26.6\% in the data set.

\begin{figure}[!t]
  \centering
  \includegraphics[width=2.9in]{content/images/hist_initial_balancing.png}
  \caption{Distribution of the initial balancing states based on the players' win rates in the generated data set of 1000 levels. We use this data set to compare the different representations.}
  \label{fig:init-balancing}
\end{figure}

To evaluate the performance of the balancing method we compare the balancing state before and after per representation. A general overview is given in Table~\ref{tab-overview}. A histogram of the balancing improvement is depicted in Figure~\ref{fig:repr-compare}. 

The performance of all three swap representations is at comparable quality. Each representation managed to improve the share of balanced levels significantly. The swap-narrow and swap-wide representations perform slightly better towards balancing in contrast to swap-turtle.
The plain PCGRL narrow representation also improved the share of balanced levels, however, with 36.7\% this share is smaller compared to the swap representations. Additionally, a proportion of 38.8\% of the levels are in an unplayable state at episode end~(Figure~\ref{fig:narrow-pcgrl}); whereas our methods result in 100\% of playable levels in all cases on this domain.
In all results, however, remain unbalanced levels. The biggest share remains for the balancing states 0 and 1.
\hl{For representations with a higher proportion of balanced levels, the average episode lengths are shorter. This is because levels that remain unbalanced will max out the episode length.}

%\begin{figure}[!t]
 % \centering
 % \includegraphics[width=3.5in]{content/images/repr_compare.png}
 % \caption{Comparison of balancing distributions of the balancing states before and after the balancing method per each representation. The same data set of of 1000 levels is used each time.}
%  \label{fig:repr-compare}
%\end{figure}



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
          \centering
          \includegraphics[width=\textwidth]{content/images/repr_compare.png}
          \caption{\normalfont Swap representations}
          \label{fig:repr-compare}
     \end{subfigure}
     \vspace{\fill}
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{content/images/result_narrow_pcgrl.png}
         \caption{\normalfont Original PCGRL (narrow)}
         \label{fig:narrow-pcgrl}
     \end{subfigure}
    
          \caption{Comparison of balancing state distributions before and after the balancing process per each representation using the data set of 1000 levels (Figure~\ref{fig:init-balancing}). The swap representations (a) are compared to the original PCGRL implementation directly~(b).}
     \label{fig:repr-compare}
\end{figure}



%\begin{table}[]
%\centering
%caption{Performance overview of the representations. Initially balanced levels were not taken into account.}
%\label{tab-overview}
%\begin{tabular}{@{}lllll@{}}
%\toprule
%                        & Swap-narrow  & Swap-turtle   & Swap-wide    & PCGRL        \\ \midrule
%Balanced (\%)           & \textbf{48.1}   & 42.5          & \textbf{48.1}  & 30.4    \\
%Improved (\%)           & 63.3         & 56.8          & \textbf{64.1}    & 36.7      \\
%Playable (\%)           & 100          & 100           & 100            & 61.2      \\
%Avg. changes            & 4.6$\pm$1.9  & 4.7$\pm$1.9   & 4.9$\pm$1.9  & 5$\pm$1.8    \\
%Avg. ep. length         & 11.3$\pm$6.1 & 25.4$\pm$17.7 & 14.1$\pm$7.9 & 15$\pm$7.9   \\
%Size action space       & 2            & 32            & 2592         & 10           \\
%Compute time (h)       & \textbf{52}   & 40              & 33            &  \\
%\bottomrule
%\end{tabular}
%\end{table}


\begin{table}[btp]
\caption{Performance overview of the representations. Initially balanced levels were not taken into account.}
\begin{center}
\begin{tabular}{l|l|l|l|l}
                        & {\textbf{S-narrow$^{\mathrm{*}}$}}  & {\textbf{S-turtle$^{\mathrm{*}}$}} & {\textbf{S-wide$^{\mathrm{*}}$}} & {\textbf{PCGRL}}   \\
\hline
Balanced (\%)           & \textbf{48.1}   & 42.5          & \textbf{48.1}  & 30.4    \\
Improved (\%)           & 63.3         & 56.8          & \textbf{64.1}    & 36.7      \\
Avg. changes            & 4.6$\pm$1.9  & 4.7$\pm$1.9   & 4.9$\pm$1.9  & 5$\pm$1.8    \\
Avg. ep. length         & 11.3$\pm$6.1 & 25.4$\pm$17.7 & 14.1$\pm$7.9 & 15$\pm$7.9   \\
Size action space            & 2            & 32            & 2592         & 10           \\
\multicolumn{2}{l}{} \\
\multicolumn{4}{l}{$^{\mathrm{*}}$Swap representations are abbreviated with S.}
\end{tabular}
\label{tab-overview}
\end{center}
\end{table}


\subsection{Generated levels}
\label{sec:gen-levels}
Figure \ref{fig:gen-level1} and \ref{fig:gen-levels} give examples of the different types of generated levels taken from the samples in Section \ref{sec:eval-swap}. Figure \ref{fig:res-perfect} is an example where the balancing agent altered the given level to a balanced level by swapping only one tile. By swapping the highlighted grass tile with the rock tile the path to the resource (forest) tiles is now blocked. This results in a more equal availability of food resources for both players. In Figure \ref{fig:gen-level1} the agent balanced the level from an initial balancing state of 0.3 to 0.5. By swapping the marked water tile to a more central position for both players, the balancing is improved. In Figure \ref{fig:res-failed} the agent failed to balance the initial level with $b_0=0$. The balancing process terminated after the maximum of permitted changes has been reached. In the end $b$ is still 0.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.41\textwidth}
         \centering
         \includegraphics[width=58mm]{content/images/res_perfect2.png}
         \caption{\normalfont The agent balanced a maximally unbalanced level (0) towards a balanced level (0.5) by swapping one tile.}
         \label{fig:res-perfect}
     \end{subfigure}
      \vspace{\fill}
     \begin{subfigure}[b]{0.41\textwidth}
         \centering
         \includegraphics[width=58mm]{content/images/res_nochange2.png}
         \caption{\normalfont The agent could not change the initial balancing of 0. Generation stopped after a permitted number of changes has been exceeded. Since several tiles have been swapped, they are not highlighted for the sake of visualization.}
         \label{fig:res-failed}
     \end{subfigure}
    
    \caption{Examples of altered levels by the balancing agent. The left column shows generated levels before balancing. The right level is the result after the balancing process. Swapped tiles are indicated by red frames.}
     \label{fig:gen-levels}
\end{figure}

\subsection{Impact of tiles on balancing}
\label{sec:impact}
The analysis of the actual swaps a model made gives insights on its behavior. Thus, we showed the model could improve the balancing state of the given levels, we can further argue that swaps made by the model have impact on the balancing. In reverse, we can conclude from this behavior which tiles in the game have most impact on balancing.

For comparison, we calculate per swap pair the relative differences of frequencies of random swaps with the ones from the models. Therefore, these frequencies are factorized with the inverse probabilities of total tile occurrences in the data set. Due to swapping the same tile types is prohibited by the representations, ten different combinations are possible. This is depicted in Figure~\ref{fig:swaps}.
The figure shows the three representations have different behaviors; however, they agree in particular points. Most impact has the swapping of forest with stone tiles, second the swap of forest with water tiles. This makes sense in the context of the resource gathering win condition. Relocating the resource tiles forest or water will likely affect the balancing state thus, they are included in the win condition.
A stone field can be used to block the way for players. Due to this, the swapping of forest with stone tiles has an additional powerful impact.
Surprisingly swapping players' spawn positions is not a favored action in all cases.


\begin{figure}[!t]
  \centering
  \includegraphics[width=3.5in]{content/images/swap-analysis2.png}
  \caption{Comparing the swapped tiles by the model per representation on the generated 1000 levels. The comparison is made in relation to the inverse tile type distribution of all levels. This shows the difference to random swapping.}
  \label{fig:swaps}
\end{figure}


\section{Extended study on general improvements and balancing with a varied target balance}
\label{sec:extensions}

In Section~\ref{sec:experiments} we focused on a balancing where both players win equally often. This study extends the paper's core idea to demonstrate that this method is capable of optimizing given levels towards arbitrary balancing values as well. Furthermore, the performances of the trained models are improved.

\subsection{Improvement of results}
\label{sec:improvements}

To improve the results from Section~\ref{sec:experiments}, we addressed two issues:
First, previously both players' spawn positions were represented by the same type of tile, making it impossible for the model to distinguish.
For this reason, we are now assigning different tile representations to each spawn position, as our previous research has shown that these affect balancing.
The different encoding of both positions adds more information and thus slightly increases the observation space, but the action space remains the same.

Second, we have improved the performance of the code, which reduces the computation time. This made training more efficient while also resulting in more updates \hl{(10k)} of the model's policy within the same time.

In the results of the experiments in Table~\ref{tab-overview}, the best model could balance 48.1\% and could improve 64.1\% of the levels towards the desired balancing of 0.5. In this extended work, we improve the proportion of balanced levels to 68\% compared to this baseline (Table~\ref{tab:unbalancing}). The levels where the model could at least improve towards the desired balancing are improved to a proportion of 88.9\%. \hl{A level is considered improved if the balancing is equal or comes closer to the desired state.}

\subsection{Balancing with different target values}
\label{sec:unbalancing}
With this experiment series we expand the previous research towards also training models to generate levels which are not balanced equally for both players. This shows, that our method is capable of balancing levels to a distinct value in general.

Therefore, we use the adjusted reward function (Eq.~\ref{eq:reward}) which is configurable with a parameter $b$ towards a desired balancing. We investigate this by training \hl{six} different models in tenth increments of possible values for $b$ \hl{in the interval $[0,0.5]$.} As it performed best according to the previous results we use the swap-wide representation in combination with the improvements from Section~\ref{sec:improvements}. \hl{We refrain from implementing a single but controllable approach as in}~\cite{earle_learning_2021}, \hl{as we experiment with different parametrizations of the reward function only. Applying controllable RL would mean an adaption of the previously defined MDP, making a direct comparison with the previous results difficult.}
To evaluate all models, we use the same level data set from Section~\ref{sec:eval-swap} to ensure comparability. An overview of the results is given in Table~\ref{tab:unbalancing}.
%Figure~\ref{fig:unbalancing}.

For all values of $b$, a significant improvement of the respective balancing state can be observed (blue). The performance, however, differs depending on $b$. For \hl{$b \geq 0.3$} the proportion of levels with the desired balancing is even higher than the baseline from the previous experiments. For the value 0 indicating levels being heavily balanced towards one specific player the performance is slightly worse than the baseline. In all cases, however, the models could improve the balancing towards the given value significantly.

\hl{Through matrix comparisons, we determined for each $b$ a content diversity of 100\% of the balanced levels. This works aims to generate asymmetrical yet balanced levels. To evaluate this, we checked all levels for each model, considering both diagonals as well as the vertical and horizontal axes. None of the levels created had any form of symmetry.
Both, the checking of diversity and symmetry are solutions at the value layer, however, not at the semantic one. There may be levels that are semantically the same e.g., if only a few tiles are different, which have no influence on the game. This process, however, cannot be easily automated. 
%No semantically identical or symmetrical levels were found when manually examining a random subset of 25.
}

\begin{table}
    \centering
    \caption{\hl{Performance overview of six swap-wide models trained to optimize different balancing values $b$ across the interval $[0,0.5]$ of the balancing metric} (cf. Section~\ref{sec:reward}). All values are expressed as percentages.}
    \begin{tabular}{c|c|c|c|c}
         $b$ &  \textbf{Balanced to $b$}&  \textbf{Improved toward $b$} & \textbf{Initial $=b$} & \textbf{Baseline} \\ \hline
         0.0&  36.1&  71.1&  8.6& -\\
         0.1&  35.1&  73.5&  7.2& -\\
         0.2&  42.9&  76.3&  6.4& -\\
         0.3&  54.6&  77.9&  11.4& -\\
         0.4&  60.7&  81.4&  12.0& -\\
         0.5&  \textbf{68.0} &  88.9&  15.6& 48.1\\
    \end{tabular}
    \label{tab:unbalancing}
\end{table}


%\begin{figure*}[!t]
%  \centering
%  \includegraphics[width=0.75\linewidth]{content/images/unbalancing_overview.png}
%  \caption{Performance overview of eleven swap-wide models trained to optimize different balancing values $b$ across the interval $[0,1]$ of the balancing metric (cf. Section~\ref{sec:reward}). The plot shows the improvement of the proportion of the levels which are initially in the desirable state (red) to the proportion after the balancing proceeding (blue). The green line represents the proportion of levels where the models could at least improve the balancing value towards the desired goal. For all results, levels which are already in the desired balancing state have been filtered out. As a baseline, the previous result from Section~\ref{sec:experiments} is shown~(orange).}
%  \label{fig:unbalancing}
%\end{figure*}

%\section{Extended study on adding more player agents}

%\subsection{Reward design for n-players}
%\begin{equation}
%\label{eq:new-bt}
%wr_{p,t} = \frac{1}{wl_t} \sum_{i=1}^{w_{p,t}} w_{p,t,i}
%\end{equation}


%\begin{equation}
%\label{eq:new-bt}
%b_t = \sum_{p=1}^{P} | wr_{p,t}-\frac{1}{P} |
%\end{equation}

%\subsection{Level generator for N players}

%\subsection{Direct comparison of the old reward function with new function}

%\subsection{Experiments and Results}




\section{Discussion and limitations}
\label{sec:discussion}
% In this work, we proposed a method for automated level balancing with RL. We showed our method using swap-based representations performs better within less training steps compared to the original PCGRL.
Our experiments showed promising results within fewer training steps compared to the original PCGRL while being more robust to ensure playability. There are, however, several things that need to be discussed.

The reward of the balancing agent represents the balancing state of multiple simulations on the current level state. By design, this is done with the use of the information of which player actually won per simulation pass. Using game specific information such as e.g., the health state of players inside the reward function potentially might improve the results. This is, however, not desired since including domain specific information creates dependencies on the distinct game. In this case, a special reward function must be developed for each game. Furthermore, including too much or the wrong information could bias the reward resulting in poor performance or unwanted behavior of the model. As a consequence, the model would not learn what \emph{really} influences balancing, or it might exploit unforeseen loopholes.


Splitting up the level generation and balancing process into separated units yielded much better results than doing it in the same step as in the original PCGRL. 
The plain PCGRL might be able to achieve comparable results when trained significantly longer, however, the here proposed architecture converges faster in less updates of the policy. This gives evidence that our architecture is more efficient by subdividing the problem into two simpler problems. In combination with the swapping representations, the balancing process can fully focus on balancing. We compared three adapted representations from the original PCGRL and evaluated them regarding performance. All of them can improve the balancing state, whereas swap-turtle yielded slightly worse results than the other two. Thus, swap-narrow, and swap-wide perform comparably, we recommend using the narrow representation when faster training and generation is required. It is, furthermore, independent from the grid size. If the focus is on performance we recommend using the swap-wide representation.
%\hl{Through matrix comparisons, we determined a content diversity of 100\% of the generated and balanced levels. This is a solution at the value layer, however, not at the semantic one. There may be levels that are semantically the same e.g., if a few tiles are different, which has no influence on the game. This process cannot be easily automated. A manual examination of a random subset of 50, no semantically identical levels could be found.}

Since we showed, that the model improves a level's balancing significantly, it is possible to draw conclusions about which tile types have most impact on balancing regarding their swap-frequencies.
For this domain, the swapping of resource tiles (e.g., forest) with blocking elements (stone) had the greatest impact. \hl{Swapping players' spawn position was not a favored action. We assume that this is due to the small number of available types of this type (only two) compared to resource tiles and therefore the model had less experience in learning these swaps appropriately.}

By simulating the game $n$-times with player agents the balancing state is evaluated. This metric is of course dependent on exactly these types of players. \hl{In online gaming, the pairing of players of the same skills is often ensured through matchmaking algorithms}~\cite{alman_theoretical_2017}\hl{ that utilize the Elo-rating system}~\cite{elo_rating_1978}.
For players with e.g., different skill or type the balancing would be different. That is a limitation, however, being also an advantage. By using different types of player agents, the game level could be balanced to compensate skill differences of the players by solely adjusting the level not the players themselves. This is of high interest when balancing levels for different player types such as a mage and a fighter. It can be applied in e.g.; role play games where gear levels are an indicator of the character strength. So, players can use their long-farmed equipment in a competitive setting and the game could be balanced through the environment only. In future research, our work is to be extended towards this. The controllable content generators~\cite{earle_learning_2021} might be an applicable solution in that context.

An issue of the proposed architecture is a computational effort in the training of the model which lies in the simulation step for rewarding. For each swap the agent takes on the level the simulation step is run. As it learns in training, this is the reason why RL is an appropriate method to apply here. In contrast, e.g., an evolutionary approach would need unnecessary steps of evaluating its fitness since it starts over again each time from scratch. 
In addition, we figured out that the reward is mostly sparse in training. That indicates, only a small sub sample of the action space are actually actions which influence the balancing. Especially in the beginning of the training, this must be learnt by the model first.
In order to speed up the training process, we are considering methods that reduce the computational effort. This would also be of great interest for the application in more complex environments.
One solution might be to reward the agent after several time steps only or even use sparse rewards. Despite the learning process would then be harder for the agent, simulation steps for the reward are omitted. Thus, the training process is sped up and the agent can explore faster.
\hl{Another approach could be the usage of a surrogate reward model to predict a level's balancing state. This would speed up training a lot, however, the model's accuracy must be high enough to give appropriate rewards to ensure a correct training. Lowering the reward calculation costs thereby improves the feasibility of an evolutionary algorithm. Investigating the swap-based representation pattern incorporated into the crossovers or mutations of an evolutionary algorithm represents an interesting target for future research.}

\subsection{Discussion on the application of fairness metrics for game balancing}
We've automated the decision-making process of how balanced a game is, based on a function inspired from the Statistical Parity metric~\cite{dwork_fairness_2012}.
This metric is commonly used in the fair machine learning community for e.g., to measure how fair automated decision-making systems based on machine learning are~\cite{makhlouf_applicability_2021}. With this section, we want to open the discussion on how fairness metrics can be applied to game balancing in general. At this point, it is important to mention, that the concept of fairness is a social and ethical concept and not a statistical~\cite{chouldechova_fair_2017}. Games are, however, designed to be played by humans. Therefore, social and ethical considerations should be taken into account when applying an automated balancing process, particularly in a competitive environment with multiple players.

\paragraph{\hl{An acceptable range of win rates}} So far, we only considered the balancing proceeding for a level as success if the metric corresponded exactly to the predefined balancing goal (e.g., $b=0.5$). An exact measuring of a certain value through sampling is, however, in many cases not achievable. Although we have examined how often we should sample to find a balance between the number of simulation runs and minimizing uncertainty for the estimation of the actual game balance, there is still a residual uncertainty. This is also a problem that often arises when collecting data about the real world such as surveys etc. To address this issue, a solution is the introduction of a bias and define the optimal value not as a single value, but as a range. The \emph{Disparate Impact} metric~\cite{feldman_certifying_2015,saleiro_aequitas_2018} expresses fairness with the ratio of a predicted outcome of two groups. The fairest ratio here would be represented by a value of 1. A commonly used range for this metric to consider an outcome as fair is~$>=0.8$ as stated in~\cite{saleiro_aequitas_2018}. That being said, applied to game balancing values in a range to the desired value can be considered as balanced. For this work, we could define a balanced game state as: \hl{$1-(w_{p1t} - w_{p2t}) \ge 0.8$.} Introducing this bias would increase the range of levels considered balanced, resulting in an even better proportion of balanced levels in our method. Since this bias has a strong influence on that proportion, it should be adapted to the game domain with regard to the residual uncertainty when transferred to game balancing.



\section{Conclusion and Future Work}
\label{sec:conclusion}
In this paper, we proposed a new method to balance tile-based game levels with reinforcement learning (RL).
Therefore, we introduced a novel swap-based representation family for the PCGRL framework, where the RL agent swaps the locations of tiles in a given level.
Our architecture benefits from separating the level generation and balancing process into two subsequent processes. The latter can therefore be considered as a task for fine-tuning existing content.
In this extended article we discussed the application of existing fairness metrics to game balancing and thus derived the reward function for the RL from the Statistical Parity metric, in order to automatically measure the balancing state of a level.
%and include information from simulated game runs.
Furthermore, we improved the results from the conference paper on level balancing to a proportion of balanced levels of 68\% and the proportion of improvements to 88.9\%. Compared to the original PCGRL method (30.4\%) on generated levels of the NMMO environment, our approach is easier to learn and significantly improves the results.

In addition, our approach is generalized and we have shown how one can also generate levels with a specific balance in order to generate unbalanced levels that favor a specific player. This opens new perspectives to create levels when e.g., adults play vs. children or for players with different gear levels.
Finally, by analyzing which tiles are swapped frequently, information can be inferred which tile types influence the balancing most. This provides game developers with additional empirical evidence about how the game system itself actually behaves.

For future work, we want to test our method with increased player sizes. Additionally, the balancing for players of different types like e.g., a mage versus an archer by only altering the game level is of interest. Moreover, we think that this method is applicable not only to games, but also to other domains as well. In subsequent research we are interested in the application to city planning for fair infrastructure distribution.

\section*{Acknowledgments}
We thank Christoph Kern, Frederic Gerdon, Jakob Kappenberger, and Lea Cohausz for their feedback and discussions on fairness metrics. We would also like to thank Patrick Takenaka for further feedback and comments.
